The C$^{18}$O core mass function toward Orion A: Single-dish observations

We have performed an unbiased dense core survey toward the Orion A Giant Molecular Cloud in the C$^{18}$O ($J$=1--0) emission line taken with the Nobeyama Radio Observatory (NRO) 45-m telescope. The effective angular resolution of the map is 26", which corresponds to $\sim$ 0.05 pc at a distance of 414 pc. By using the Herschel-Planck H$_2$ column density map, we calculate the C$^{18}$O fractional abundance and find that it is roughly constant over the column density range of $\lesssim$ 5 $\times$ 10$^{22}$ cm$^{-3}$, although a trend of C$^{18}$O depletion is determined toward higher column density. Therefore, C$^{18}$O intensity can follow the cloud structure reasonably well. The mean C$^{18}$O abundance in Orion A is estimated to be 5.7$\times$10$^{-7}$, which is about 3 times larger than the fiducial value. We identified 746 C$^{18}$O cores with astrodendro and classified 709 cores as starless cores. We compute the core masses by decomposing the Herschel-Planck dust column density using the relative proportions of the C$^{18}$O integrated intensities of line-of-sight components. Applying this procedure, we attempt to remove the contribution of the background emission, i.e., the ambient gas outside the cores. Then, we derived mass function for starless cores and found that it resembles the stellar initial mass function (IMF). The CMF for starless cores, $dN/dM$, is fitted with a power-law relation of $M^\alpha$ with a power index of $\alpha = -$2.25$\pm$ 0.16 at the high-mass slope ($\gtrsim$ 0.44 $M_\odot$). We also found that the ratio of each core mass to the total mass integrated along the line of sight is significantly large. Therefore, in the previous studies, the core masses derived from the dust image are likely to be overestimated at least by a factor of a few. Accordingly, such previous studies may underestimate the star formation efficiency of individual cores.

==> tables/OrionA_core_catalog.tex <==
 \\ \hline \hline 
 ID & RA & Dec & \multicolumn{1}{c}{$v_\mathrm{LSR}$} & \multicolumn{1}{c}{$A$}& \multicolumn{1}{c}{$T^*_\mathrm{mb,\ peak}$} & \multicolumn{1}{c}{$a_\mathrm{major}$}& \multicolumn{1}{c}{$a_\mathrm{minor}$} & \multicolumn{1}{c}{PA} & \multicolumn{1}{c}{$2R_\mathrm{core}$}& \multicolumn{1}{c}{$2R_\mathrm{core}$} & \multicolumn{1}{c}{$dV_\mathrm{core}$}& \multicolumn{1}{c}{$M_\mathrm{core}$} & \multicolumn{1}{c}{$M_\mathrm{vir}/M_\mathrm{core}$}& \multicolumn{1}{c}{$\overline{n}$} & \multicolumn{1}{c}{YSO}\\ 
  & (J2000) & (J2000) & \multicolumn{1}{c}{(km s$^{-1}$)} & \multicolumn{1}{c}{(arcsec$^2$)}&\multicolumn{1}{c}{(K)} & \multicolumn{1}{c}{(arcsec)}& \multicolumn{1}{c}{(arcsec)} & \multicolumn{1}{c}{(deg)} & \multicolumn{1}{c}{(arcsec)}& \multicolumn{1}{c}{(pc)} & \multicolumn{1}{c}{(km s$^{-1}$)}& \multicolumn{1}{c}{($M_\odot$)} &   & \multicolumn{1}{c}{(10$^4$ cm$^{-3}$)} &  \\ 
 \hline \\ \endfirsthead 
 \caption[]{Continued} \\ 
 \hline \hline 
 ID & RA & Dec & \multicolumn{1}{c}{$v_\mathrm{LSR}$} & \multicolumn{1}{c}{$A$}& \multicolumn{1}{c}{$T^*_\mathrm{mb,\ peak}$} & \multicolumn{1}{c}{$a_\mathrm{major}$}& \multicolumn{1}{c}{$a_\mathrm{minor}$} & \multicolumn{1}{c}{PA} & \multicolumn{1}{c}{$2R_\mathrm{core}$}& \multicolumn{1}{c}{$2R_\mathrm{core}$} & \multicolumn{1}{c}{$dV_\mathrm{core}$}& \multicolumn{1}{c}{$M_\mathrm{core}$} & \multicolumn{1}{c}{$M_\mathrm{vir}/M_\mathrm{core}$}& \multicolumn{1}{c}{$\overline{n}$} & \multicolumn{1}{c}{YSO}\\ 
  & (J2000) & (J2000) & \multicolumn{1}{c}{(km s$^{-1}$)} & \multicolumn{1}{c}{(arcsec$^2$)}&\multicolumn{1}{c}{(K)} & \multicolumn{1}{c}{(arcsec)}& \multicolumn{1}{c}{(arcsec)} & \multicolumn{1}{c}{(deg)} & \multicolumn{1}{c}{(arcsec)}& \multicolumn{1}{c}{(pc)} & \multicolumn{1}{c}{(km s$^{-1}$)}& \multicolumn{1}{c}{$M_\odot$} &   & \multicolumn{1}{c}{(10$^4$ cm$^{-3}$)} &  \\ 
 \hline \\ \endhead 
 1 & 5 33 44.7 & 5 18 5 & 72.9 & 5738 & 1.7 & 21.8 & 19.3 & -149 & 85.5 & 0.17 & 0.38 & 1.42 & 0.33 & 0.95 & N \\ 
 2 & 5 33 45.0 & 5 24 24 & 61.9 & 2756 & 2.9 & 25.0 & 10.8 & 89 & 59.2 & 0.12 & 0.18 & 0.32 & 0.23 & 0.64 & N \\ 
 3 & 5 33 47.3 & 5 19 48 & 62.7 & 2925 & 1.5 & 30.8 & 8.9 & 84 & 61.0 & 0.12 & 0.17 & 0.43 & 0.16 & 0.80 & N \\ 
 4 & 5 33 48.2 & 5 29 20 & 58.9 & 5119 & 3.5 & 34.1 & 9.1 & 61 & 80.7 & 0.16 & 0.28 & 1.27 & 0.19 & 1.01 & N \\ 
 5 & 5 33 48.7 & 5 45 29 & 57.0 & 2925 & 1.4 & 20.5 & 13.6 & 74 & 61.0 & 0.12 & 0.22 & 0.52 & 0.21 & 0.96 & N \\ 
 6 & 5 33 51.5 & 5 35 7 & 59.7 & 8100 & 2.9 & 24.3 & 20.3 & -175 & 101.6 & 0.20 & 0.34 & 3.33 & 0.13 & 1.33 & N \\ 
 7 & 5 33 51.9 & 5 10 15 & 84.7 & 2756 & 1.9 & 16.2 & 11.1 & 80 & 59.2 & 0.12 & 0.25 & 0.50 & 0.27 & 1.01 & N \\ 
 8 & 5 33 52.2 & 5 17 8 & 81.6 & 3263 & 1.6 & 24.3 & 12.5 & -138 & 64.5 & 0.13 & 0.19 & 1.17 & 0.07 & 1.83 & N \\ 
 9 & 5 33 52.6 & 5 28 36 & 63.4 & 2475 & 3.3 & 27.9 & 8.9 & 59 & 56.1 & 0.11 & 0.25 & 0.48 & 0.28 & 1.13 & N \\ 
 10 & 5 33 53.4 & 5 32 17 & 60.4 & 5794 & 2.8 & 23.7 & 15.1 & 145 & 85.9 & 0.17 & 0.34 & 1.65 & 0.23 & 1.09 & N \\ 
 11 & 5 33 53.6 & 5 19 6 & 70.1 & 2250 & 2.7 & 16.1 & 10.2 & 85 & 53.5 & 0.11 & 0.19 & 0.29 & 0.26 & 0.80 & N \\ 
 12 & 5 33 53.8 & 5 21 39 & 62.6 & 6581 & 4.1 & 39.4 & 10.7 & 87 & 91.5 & 0.18 & 0.30 & 1.49 & 0.20 & 0.81 & N \\ 
 13 & 5 33 54.9 & 5 11 42 & 86.7 & 4838 & 2.0 & 22.0 & 11.4 & 56 & 78.5 & 0.16 & 0.77 & 1.07 & 1.65 & 0.92 & N \\ 
 14 & 5 33 55.1 & 5 19 10 & 76.8 & 2250 & 1.6 & 17.8 & 10.1 & 46 & 53.5 & 0.11 & 0.27 & 0.16 & 0.94 & 0.45 & N \\ 
 15 & 5 33 56.5 & 5 9 40 & 86.8 & 6694 & 1.8 & 44.4 & 13.8 & 59 & 92.3 & 0.19 & 0.37 & 1.78 & 0.26 & 0.94 & N \\ 
 16 & 5 33 58.0 & 5 23 57 & 61.6 & 3769 & 5.0 & 23.4 & 10.1 & 88 & 69.3 & 0.14 & 0.22 & 2.55 & 0.05 & 3.20 & Y \\ 
 17 & 5 33 59.9 & 5 28 29 & 59.4 & 4444 & 5.1 & 20.6 & 12.6 & 117 & 75.2 & 0.15 & 0.29 & 2.17 & 0.11 & 2.13 & N \\ 
 18 & 5 34 1.0 & 5 26 43 & 65.3 & 3488 & 3.5 & 19.7 & 11.1 & 72 & 66.6 & 0.13 & 0.22 & 0.92 & 0.14 & 1.29 & N \\ 
 19 & 5 34 1.9 & 5 4 11 & 88.1 & 36563 & 1.9 & 53.6 & 40.1 & 117 & 215.8 & 0.43 & 0.72 & 12.55 & 0.34 & 0.52 & N \\ 
 20 & 5 34 3.0 & 5 32 3 & 62.3 & 10294 & 4.8 & 61.3 & 15.8 & 71 & 114.5 & 0.23 & 0.38 & 6.85 & 0.09 & 1.91 & N \\ 
 21 & 5 34 4.3 & 5 35 33 & 63.7 & 2419 & 4.0 & 22.2 & 9.1 & 99 & 55.5 & 0.11 & 0.22 & 0.95 & 0.11 & 2.33 & N \\ 
 22 & 5 34 4.9 & 5 28 17 & 63.6 & 3038 & 2.5 & 14.7 & 12.4 & -140 & 62.2 & 0.12 & 0.32 & 0.63 & 0.39 & 1.09 & N \\ 
 23 & 5 34 5.9 & 5 29 23 & 61.0 & 2925 & 2.0 & 13.4 & 13.1 & -168 & 61.0 & 0.12 & 0.34 & 0.73 & 0.37 & 1.34 & N \\ 
 24 & 5 34 7.8 & 5 36 24 & 74.2 & 4556 & 1.4 & 29.4 & 14.5 & -137 & 76.2 & 0.15 & 0.18 & 0.42 & 0.22 & 0.40 & N \\ 
 25 & 5 34 8.3 & 4 53 28 & 73.3 & 11644 & 3.0 & 43.7 & 22.1 & 63 & 121.8 & 0.24 & 0.37 & 2.99 & 0.21 & 0.69 & N \\ 
 26 & 5 34 9.6 & 5 32 15 & 60.9 & 2644 & 2.5 & 19.0 & 9.2 & 155 & 58.0 & 0.12 & 0.26 & 0.70 & 0.21 & 1.51 & N \\ 
 27 & 5 34 10.5 & 5 37 9 & 61.8 & 6075 & 3.7 & 31.4 & 18.3 & 176 & 87.9 & 0.18 & 0.36 & 2.40 & 0.18 & 1.48 & N \\ 
 28 & 5 34 11.9 & 5 28 39 & 70.7 & 8269 & 1.9 & 38.1 & 22.1 & 157 & 102.6 & 0.21 & 0.48 & 1.07 & 0.86 & 0.41 & N \\ 
 29 & 5 34 12.4 & 5 30 41 & 71.6 & 5569 & 1.6 & 31.4 & 16.9 & 113 & 84.2 & 0.17 & 0.31 & 0.93 & 0.33 & 0.65 & N \\ 
 30 & 5 34 12.5 & 4 55 31 & 82.9 & 3488 & 1.4 & 35.1 & 9.8 & 104 & 66.6 & 0.13 & 0.15 & 0.29 & 0.19 & 0.41 & N \\ 
 31 & 5 34 12.6 & 5 0 15 & 84.6 & 8325 & 1.5 & 30.0 & 21.1 & -149 & 103.0 & 0.21 & 0.45 & 2.41 & 0.33 & 0.92 & N \\ 
 32 & 5 34 14.3 & 5 28 29 & 61.4 & 3825 & 2.2 & 19.0 & 12.3 & 164 & 69.8 & 0.14 & 0.28 & 0.67 & 0.32 & 0.82 & N \\ 
 33 & 5 34 15.0 & 5 33 0 & 57.4 & 4669 & 2.2 & 21.1 & 16.5 & 162 & 77.1 & 0.15 & 0.29 & 0.93 & 0.26 & 0.85 & N \\ 
 34 & 5 34 15.1 & 5 2 13 & 85.2 & 13950 & 1.5 & 64.4 & 20.0 & -143 & 133.3 & 0.27 & 0.40 & 3.69 & 0.21 & 0.65 & N \\ 
 35 & 5 34 15.8 & 5 37 49 & 78.2 & 5513 & 1.6 & 28.0 & 16.5 & 134 & 83.8 & 0.17 & 0.17 & 0.60 & 0.15 & 0.43 & N \\ 
 36 & 5 34 16.4 & 5 34 58 & 55.3 & 2475 & 2.1 & 14.9 & 10.7 & -139 & 56.1 & 0.11 & 0.22 & 0.54 & 0.20 & 1.26 & N \\ 
 37 & 5 34 17.0 & 5 29 6 & 68.1 & 2925 & 2.4 & 17.6 & 10.9 & 85 & 61.0 & 0.12 & 0.20 & 0.51 & 0.19 & 0.94 & N \\ 
 38 & 5 34 17.1 & 5 36 44 & 56.4 & 7706 & 5.2 & 25.3 & 21.0 & -172 & 99.1 & 0.20 & 0.37 & 5.51 & 0.09 & 2.37 & N \\ 
 39 & 5 34 17.5 & 5 34 43 & 60.0 & 1856 & 2.0 & 17.7 & 8.4 & 178 & 48.6 & 0.10 & 0.20 & 0.39 & 0.20 & 1.40 & N \\ 
 40 & 5 34 17.6 & 5 26 49 & 62.8 & 6356 & 2.6 & 40.4 & 14.5 & 128 & 90.0 & 0.18 & 0.35 & 1.47 & 0.29 & 0.84 & N \\ 
 41 & 5 34 18.0 & 5 14 14 & 84.5 & 6075 & 1.4 & 29.8 & 15.4 & 172 & 87.9 & 0.18 & 0.31 & 2.05 & 0.15 & 1.26 & N \\ 
 42 & 5 34 18.2 & 4 53 42 & 76.6 & 5569 & 2.1 & 20.2 & 19.4 & -138 & 84.2 & 0.17 & 0.30 & 1.44 & 0.20 & 1.01 & N \\ 
 43 & 5 34 18.2 & 5 27 6 & 68.5 & 2925 & 2.4 & 18.7 & 10.4 & 104 & 61.0 & 0.12 & 0.25 & 0.94 & 0.15 & 1.74 & N \\ 
 44 & 5 34 18.6 & 5 30 13 & 64.8 & 2531 & 2.6 & 15.4 & 11.1 & 51 & 56.8 & 0.11 & 0.25 & 0.68 & 0.19 & 1.56 & N \\ 
 45 & 5 34 20.8 & 5 41 9 & 80.8 & 5119 & 1.6 & 24.6 & 15.2 & 151 & 80.7 & 0.16 & 0.35 & 1.91 & 0.20 & 1.52 & N \\ 
 46 & 5 34 20.9 & 5 43 42 & 74.9 & 10744 & 2.9 & 28.9 & 21.7 & 102 & 117.0 & 0.23 & 0.45 & 4.13 & 0.21 & 1.08 & N \\ 
 47 & 5 34 21.0 & 5 38 11 & 60.1 & 10181 & 3.9 & 34.3 & 18.2 & -176 & 113.9 & 0.23 & 0.83 & 8.44 & 0.35 & 2.39 & N \\ 
 48 & 5 34 21.8 & 5 20 23 & 73.6 & 11700 & 1.8 & 31.2 & 22.3 & 108 & 122.1 & 0.24 & 0.52 & 2.74 & 0.45 & 0.63 & N \\ 
 49 & 5 34 22.3 & 4 56 57 & 76.0 & 7425 & 2.5 & 36.8 & 14.9 & 133 & 97.2 & 0.20 & 0.31 & 1.63 & 0.22 & 0.74 & N \\ 
 50 & 5 34 23.0 & 5 3 9 & 75.6 & 9675 & 1.7 & 32.7 & 19.7 & -154 & 111.0 & 0.22 & 0.26 & 3.96 & 0.07 & 1.21 & N \\ 
 51 & 5 34 23.1 & 5 30 18 & 75.8 & 7369 & 1.4 & 47.8 & 17.1 & 74 & 96.9 & 0.19 & 0.27 & 1.22 & 0.21 & 0.56 & N \\ 
 52 & 5 34 23.4 & 5 33 15 & 77.1 & 1688 & 1.6 & 11.5 & 8.7 & 137 & 46.4 & 0.09 & 0.15 & 0.24 & 0.17 & 1.02 & N \\ 
 53 & 5 34 24.0 & 5 6 56 & 81.1 & 7650 & 1.6 & 24.0 & 21.4 & 92 & 98.7 & 0.20 & 0.49 & 2.70 & 0.34 & 1.17 & N \\ 
 54 & 5 34 24.0 & 5 45 47 & 70.6 & 2925 & 2.6 & 13.7 & 11.7 & 68 & 61.0 & 0.12 & 0.35 & 0.88 & 0.32 & 1.62 & N \\ 
 55 & 5 34 24.2 & 5 29 55 & 67.5 & 7875 & 1.5 & 34.9 & 15.4 & 77 & 100.1 & 0.20 & 0.33 & 2.17 & 0.19 & 0.90 & N \\ 
 56 & 5 34 24.6 & 5 26 45 & 63.4 & 1069 & 2.7 & 8.7 & 6.7 & -138 & 36.9 & 0.07 & 0.36 & 0.28 & 0.64 & 2.32 & N \\ 
 57 & 5 34 24.7 & 5 19 45 & 62.6 & 7819 & 2.3 & 28.7 & 16.6 & 121 & 99.8 & 0.20 & 0.42 & 2.22 & 0.30 & 0.93 & N \\ 
 58 & 5 34 24.7 & 5 22 5 & 70.3 & 4050 & 1.6 & 26.2 & 13.9 & 56 & 71.8 & 0.14 & 0.22 & 0.70 & 0.19 & 0.79 & N \\ 
 59 & 5 34 26.1 & 5 35 44 & 56.7 & 2869 & 4.1 & 17.8 & 10.1 & 80 & 60.4 & 0.12 & 0.33 & 1.56 & 0.16 & 2.95 & N \\ 
 60 & 5 34 26.3 & 4 51 18 & 102.2 & 4669 & 1.9 & 23.4 & 16.9 & 138 & 77.1 & 0.15 & 0.19 & 0.76 & 0.13 & 0.70 & N \\ 
 61 & 5 34 26.4 & 5 33 58 & 58.4 & 2588 & 4.8 & 15.3 & 10.1 & 108 & 57.4 & 0.12 & 0.19 & 1.28 & 0.06 & 2.83 & N \\ 
 62 & 5 34 26.6 & 5 50 17 & 76.3 & 4894 & 2.8 & 18.4 & 15.8 & 111 & 78.9 & 0.16 & 0.28 & 1.82 & 0.12 & 1.55 & N \\ 
 63 & 5 34 27.1 & 5 25 11 & 60.1 & 7819 & 4.1 & 42.6 & 11.8 & 76 & 99.8 & 0.20 & 0.59 & 3.61 & 0.36 & 1.52 & N \\ 
 64 & 5 34 27.1 & 5 48 39 & 72.0 & 3263 & 3.4 & 17.4 & 11.7 & 162 & 64.5 & 0.13 & 0.22 & 1.17 & 0.10 & 1.82 & N \\ 
 65 & 5 34 27.2 & 5 39 19 & 59.4 & 2588 & 3.1 & 16.0 & 11.2 & -150 & 57.4 & 0.12 & 0.42 & 1.10 & 0.35 & 2.43 & N \\ 
 66 & 5 34 27.6 & 5 29 14 & 73.7 & 2869 & 1.8 & 14.5 & 12.8 & 178 & 60.4 & 0.12 & 0.18 & 0.92 & 0.08 & 1.75 & N \\ 
 67 & 5 34 27.6 & 5 55 19 & 59.9 & 8550 & 2.5 & 34.1 & 15.3 & 96 & 104.3 & 0.21 & 0.27 & 3.26 & 0.09 & 1.20 & N \\ 
 68 & 5 34 27.7 & 5 18 14 & 62.2 & 4838 & 2.1 & 20.0 & 14.7 & 164 & 78.5 & 0.16 & 0.26 & 1.17 & 0.17 & 1.01 & N \\ 
 69 & 5 34 28.2 & 4 55 0 & 78.6 & 2081 & 3.0 & 15.0 & 10.2 & 106 & 51.5 & 0.10 & 0.18 & 0.56 & 0.11 & 1.72 & Y \\ 
 70 & 5 34 28.8 & 4 51 8 & 77.0 & 2419 & 1.4 & 24.3 & 11.1 & 92 & 55.5 & 0.11 & 0.14 & 0.31 & 0.13 & 0.75 & N \\ 
 71 & 5 34 29.3 & 5 18 20 & 84.3 & 7875 & 1.4 & 26.4 & 20.9 & -146 & 100.1 & 0.20 & 0.67 & 2.10 & 0.80 & 0.88 & N \\ 
 72 & 5 34 29.7 & 5 14 3 & 88.8 & 6300 & 1.9 & 22.0 & 16.9 & 116 & 89.6 & 0.18 & 0.68 & 1.42 & 1.11 & 0.83 & N \\ 
 73 & 5 34 30.0 & 5 39 45 & 79.9 & 2869 & 1.6 & 22.9 & 10.0 & -139 & 60.4 & 0.12 & 0.34 & 0.46 & 0.59 & 0.86 & N \\ 
 74 & 5 34 30.1 & 5 52 9 & 82.1 & 10181 & 1.6 & 46.1 & 22.0 & -172 & 113.9 & 0.23 & 0.29 & 4.28 & 0.08 & 1.21 & N \\ 
 75 & 5 34 30.2 & 5 36 49 & 56.2 & 4950 & 4.1 & 26.9 & 13.0 & 66 & 79.4 & 0.16 & 0.26 & 2.06 & 0.10 & 1.72 & N \\ 
 76 & 5 34 30.4 & 5 9 51 & 93.7 & 6244 & 1.4 & 30.6 & 24.9 & 115 & 89.2 & 0.18 & 0.30 & 2.18 & 0.14 & 1.29 & N \\ 
 77 & 5 34 30.7 & 5 44 11 & 61.3 & 2194 & 1.4 & 16.4 & 10.7 & 158 & 52.9 & 0.11 & 0.18 & 0.50 & 0.12 & 1.41 & N \\ 
 78 & 5 34 31.0 & 5 46 36 & 68.2 & 5344 & 4.2 & 24.3 & 15.2 & 90 & 82.5 & 0.17 & 0.21 & 2.59 & 0.05 & 1.93 & N \\ 
 79 & 5 34 31.9 & 5 22 15 & 59.0 & 23738 & 2.9 & 40.9 & 33.2 & -177 & 173.8 & 0.35 & 0.42 & 10.11 & 0.11 & 0.80 & N \\ 
 80 & 5 34 32.5 & 5 15 26 & 87.9 & 13950 & 1.7 & 54.9 & 27.1 & 82 & 133.3 & 0.27 & 0.40 & 2.55 & 0.32 & 0.45 & N \\ 
 81 & 5 34 32.6 & 4 53 60 & 86.9 & 7763 & 2.1 & 29.5 & 14.9 & -145 & 99.4 & 0.20 & 0.63 & 1.62 & 0.92 & 0.69 & N \\ 
 82 & 5 34 33.2 & 5 29 7 & 78.2 & 5906 & 1.5 & 28.5 & 16.0 & -173 & 86.7 & 0.17 & 0.48 & 1.60 & 0.48 & 1.02 & N \\ 
 83 & 5 34 33.7 & 5 25 7 & 72.4 & 9281 & 2.9 & 34.6 & 14.4 & 49 & 108.7 & 0.22 & 0.54 & 2.33 & 0.52 & 0.76 & N \\ 
 84 & 5 34 33.8 & 5 48 54 & 70.3 & 3263 & 3.3 & 17.8 & 13.9 & -177 & 64.5 & 0.13 & 0.19 & 0.87 & 0.10 & 1.36 & N \\ 
 85 & 5 34 34.3 & 5 36 28 & 77.8 & 9844 & 2.4 & 43.3 & 17.2 & 152 & 112.0 & 0.22 & 0.50 & 1.27 & 0.85 & 0.38 & N \\ 
 86 & 5 34 34.3 & 5 40 16 & 57.1 & 4669 & 3.8 & 23.6 & 11.9 & -141 & 77.1 & 0.15 & 0.44 & 3.52 & 0.16 & 3.21 & Y \\ 
 87 & 5 34 34.4 & 5 35 51 & 58.1 & 2531 & 3.2 & 19.0 & 10.6 & 80 & 56.8 & 0.11 & 0.21 & 0.55 & 0.17 & 1.26 & N \\ 
 88 & 5 34 35.4 & 5 16 40 & 79.0 & 11419 & 2.1 & 54.7 & 15.7 & 76 & 120.6 & 0.24 & 0.56 & 3.31 & 0.44 & 0.79 & N \\ 
 89 & 5 34 36.1 & 5 25 53 & 61.1 & 2700 & 1.5 & 14.8 & 14.1 & 86 & 58.6 & 0.12 & 0.27 & 0.12 & 1.42 & 0.24 & N \\ 
 90 & 5 34 36.5 & 5 46 13 & 63.4 & 3769 & 3.7 & 33.8 & 9.8 & 156 & 69.3 & 0.14 & 0.24 & 1.48 & 0.10 & 1.87 & N \\ 
 91 & 5 34 38.4 & 5 42 19 & 73.4 & 2025 & 3.1 & 17.5 & 8.0 & 62 & 50.8 & 0.10 & 0.26 & 0.69 & 0.19 & 2.21 & N \\ 
 92 & 5 34 38.6 & 5 41 37 & 60.5 & 3713 & 3.1 & 20.1 & 17.7 & 144 & 68.8 & 0.14 & 0.27 & 1.45 & 0.13 & 1.86 & N \\ 
 93 & 5 34 39.0 & 4 53 9 & 92.3 & 10125 & 2.3 & 33.3 & 21.8 & -151 & 113.5 & 0.23 & 0.44 & 1.68 & 0.50 & 0.48 & N \\ 
 94 & 5 34 39.5 & 5 26 51 & 65.9 & 5231 & 2.6 & 32.8 & 16.1 & -143 & 81.6 & 0.16 & 0.44 & 0.88 & 0.70 & 0.67 & N \\ 
 95 & 5 34 40.7 & 5 37 48 & 60.5 & 7763 & 3.7 & 23.1 & 18.3 & 68 & 99.4 & 0.20 & 0.59 & 3.24 & 0.40 & 1.38 & N \\ 
 96 & 5 34 40.8 & 5 35 23 & 59.6 & 4331 & 2.1 & 27.0 & 12.8 & -158 & 74.3 & 0.15 & 0.25 & 1.04 & 0.16 & 1.06 & N \\ 
 97 & 5 34 40.9 & 5 28 10 & 58.7 & 2475 & 3.7 & 17.4 & 9.2 & 176 & 56.1 & 0.11 & 0.22 & 0.69 & 0.15 & 1.62 & N \\ 
 98 & 5 34 41.2 & 5 31 11 & 51.0 & 11700 & 3.9 & 38.8 & 19.3 & 77 & 122.1 & 0.24 & 0.81 & 7.90 & 0.38 & 1.82 & Y \\ 
 99 & 5 34 41.4 & 4 54 51 & 89.4 & 5738 & 2.5 & 26.1 & 13.6 & -158 & 85.5 & 0.17 & 0.44 & 1.47 & 0.43 & 0.98 & N \\ 
 100 & 5 34 41.5 & 5 50 40 & 78.9 & 6413 & 1.8 & 26.3 & 20.6 & -162 & 90.4 & 0.18 & 0.40 & 1.80 & 0.31 & 1.02 & N \\ 
 101 & 5 34 41.7 & 5 11 37 & 89.2 & 15919 & 2.5 & 41.8 & 25.1 & -151 & 142.4 & 0.29 & 0.60 & 2.51 & 0.78 & 0.36 & N \\ 
 102 & 5 34 42.3 & 5 29 8 & 73.4 & 2531 & 1.4 & 18.9 & 11.0 & -177 & 56.8 & 0.11 & 0.34 & 0.16 & 1.55 & 0.37 & N \\ 
 103 & 5 34 42.8 & 4 56 52 & 67.8 & 4219 & 1.4 & 23.2 & 15.3 & 68 & 73.3 & 0.15 & 0.32 & 0.73 & 0.40 & 0.77 & N \\ 
 104 & 5 34 43.8 & 5 41 18 & 56.0 & 1406 & 4.0 & 14.2 & 6.6 & 68 & 42.3 & 0.08 & 0.19 & 0.93 & 0.06 & 5.11 & Y \\ 
 105 & 5 34 44.0 & 5 17 38 & 91.9 & 2700 & 1.3 & 15.8 & 12.6 & 95 & 58.6 & 0.12 & 0.23 & 0.69 & 0.17 & 1.43 & N \\ 
 106 & 5 34 44.3 & 6 18 30 & 102.1 & 3206 & 1.5 & 20.2 & 12.7 & 143 & 63.9 & 0.13 & 0.21 & 0.44 & 0.25 & 0.70 & N \\ 
 107 & 5 34 44.6 & 5 45 15 & 56.7 & 1800 & 3.1 & 13.0 & 8.2 & 155 & 47.9 & 0.10 & 0.24 & 0.60 & 0.17 & 2.27 & N \\ 
 108 & 5 34 44.7 & 5 29 4 & 61.9 & 6075 & 3.7 & 26.0 & 19.3 & 167 & 87.9 & 0.18 & 0.25 & 1.49 & 0.14 & 0.91 & N \\ 
 109 & 5 34 44.7 & 6 27 55 & 61.3 & 1969 & 1.9 & 14.4 & 8.9 & 122 & 50.1 & 0.10 & 0.22 & 0.34 & 0.26 & 1.14 & N \\ 
 110 & 5 34 45.2 & 5 47 37 & 73.4 & 4331 & 4.3 & 21.3 & 12.2 & 50 & 74.3 & 0.15 & 0.25 & 2.40 & 0.07 & 2.45 & N \\ 
 111 & 5 34 45.9 & 6 17 48 & 55.1 & 2813 & 1.5 & 19.9 & 10.5 & -135 & 59.8 & 0.12 & 0.36 & 0.48 & 0.63 & 0.93 & N \\ 
 112 & 5 34 46.1 & 5 49 46 & 52.5 & 9394 & 2.4 & 30.3 & 18.7 & 54 & 109.4 & 0.22 & 0.63 & 1.90 & 0.85 & 0.61 & N \\ 
 113 & 5 34 46.8 & 4 50 41 & 52.5 & 2644 & 1.5 & 19.4 & 13.2 & -141 & 58.0 & 0.12 & 0.24 & 0.53 & 0.25 & 1.14 & N \\ 
 114 & 5 34 47.2 & 5 15 34 & 77.4 & 9169 & 2.1 & 31.1 & 17.6 & 128 & 108.0 & 0.22 & 0.62 & 2.16 & 0.73 & 0.72 & N \\ 
 115 & 5 34 47.3 & 4 57 26 & 95.8 & 1575 & 1.8 & 12.0 & 8.0 & -138 & 44.8 & 0.09 & 0.18 & 0.27 & 0.21 & 1.25 & N \\ 
 116 & 5 34 47.3 & 5 32 37 & 55.0 & 2419 & 2.8 & 17.5 & 9.8 & 149 & 55.5 & 0.11 & 0.17 & 0.50 & 0.12 & 1.22 & N \\ 
 117 & 5 34 47.5 & 5 37 36 & 51.1 & 1744 & 2.9 & 12.5 & 8.7 & -170 & 47.1 & 0.09 & 0.26 & 0.53 & 0.22 & 2.13 & N \\ 
 118 & 5 34 47.6 & 5 45 29 & 70.9 & 4500 & 5.7 & 28.6 & 11.7 & 143 & 75.7 & 0.15 & 0.31 & 3.15 & 0.09 & 3.03 & N \\ 
 119 & 5 34 47.8 & 5 40 21 & 44.4 & 5681 & 1.5 & 23.2 & 17.0 & -180 & 85.1 & 0.17 & 0.25 & 0.63 & 0.33 & 0.43 & N \\ 
 120 & 5 34 48.0 & 5 30 30 & 64.1 & 5906 & 3.3 & 29.3 & 12.6 & 97 & 86.7 & 0.17 & 0.44 & 1.92 & 0.33 & 1.23 & N \\ 
 121 & 5 34 48.3 & 5 40 16 & 79.7 & 2475 & 1.4 & 12.9 & 11.2 & 81 & 56.1 & 0.11 & 0.27 & 0.32 & 0.50 & 0.76 & N \\ 
 122 & 5 34 48.4 & 6 19 28 & 53.1 & 4219 & 1.4 & 30.5 & 12.5 & 101 & 73.3 & 0.15 & 0.22 & 1.12 & 0.12 & 1.19 & N \\ 
 123 & 5 34 48.9 & 4 55 33 & 85.4 & 5175 & 5.4 & 20.6 & 14.4 & -176 & 81.2 & 0.16 & 0.50 & 5.33 & 0.14 & 4.17 & N \\ 
 124 & 5 34 48.9 & 5 2 57 & 91.3 & 13894 & 1.5 & 45.3 & 24.0 & -165 & 133.0 & 0.27 & 0.48 & 3.84 & 0.31 & 0.68 & N \\ 
 125 & 5 34 49.6 & 4 53 2 & 89.0 & 5175 & 3.5 & 35.7 & 10.3 & 55 & 81.2 & 0.16 & 0.40 & 1.44 & 0.35 & 1.12 & N \\ 
 126 & 5 34 49.8 & 5 38 54 & 56.4 & 11700 & 4.8 & 30.1 & 24.7 & 162 & 122.1 & 0.24 & 0.67 & 7.90 & 0.26 & 1.82 & N \\ 
 127 & 5 34 50.3 & 5 4 13 & 83.6 & 8606 & 2.3 & 27.9 & 18.1 & -158 & 104.7 & 0.21 & 0.45 & 2.89 & 0.28 & 1.05 & N \\ 
 128 & 5 34 50.4 & 5 33 34 & 49.8 & 5344 & 3.5 & 38.4 & 10.5 & -141 & 82.5 & 0.17 & 0.45 & 1.62 & 0.38 & 1.20 & N \\ 
 129 & 5 34 50.5 & 5 47 40 & 64.4 & 2306 & 3.4 & 14.6 & 9.7 & 102 & 54.2 & 0.11 & 0.21 & 0.84 & 0.11 & 2.21 & N \\ 
 130 & 5 34 50.6 & 5 20 27 & 85.7 & 18563 & 2.1 & 58.3 & 26.8 & 74 & 153.7 & 0.31 & 0.91 & 3.97 & 1.21 & 0.46 & N \\ 
 131 & 5 34 50.8 & 5 52 49 & 71.6 & 6638 & 2.3 & 24.2 & 20.0 & 150 & 91.9 & 0.18 & 0.42 & 1.64 & 0.38 & 0.88 & N \\ 
 132 & 5 34 50.9 & 5 43 3 & 64.9 & 2138 & 4.3 & 13.4 & 9.0 & 111 & 52.2 & 0.10 & 0.49 & 1.41 & 0.34 & 4.14 & N \\ 
 133 & 5 34 51.0 & 5 9 29 & 91.1 & 11138 & 2.4 & 41.6 & 17.0 & 160 & 119.1 & 0.24 & 0.31 & 2.17 & 0.19 & 0.54 & N \\ 
 134 & 5 34 51.3 & 5 36 34 & 53.8 & 2306 & 3.7 & 14.0 & 9.0 & -138 & 54.2 & 0.11 & 0.30 & 0.90 & 0.20 & 2.37 & N \\ 
 135 & 5 34 51.7 & 5 37 56 & 46.2 & 1181 & 3.9 & 9.7 & 7.1 & 129 & 38.8 & 0.08 & 0.28 & 0.46 & 0.24 & 3.29 & N \\ 
 136 & 5 34 51.8 & 5 19 21 & 70.4 & 1800 & 2.7 & 13.3 & 7.9 & 55 & 47.9 & 0.10 & 0.33 & 0.36 & 0.56 & 1.37 & N \\ 
 137 & 5 34 52.5 & 5 23 14 & 82.5 & 5738 & 1.5 & 45.2 & 12.5 & 53 & 85.5 & 0.17 & 0.30 & 0.50 & 0.60 & 0.33 & N \\ 
 138 & 5 34 52.6 & 5 36 3 & 81.2 & 7200 & 1.8 & 35.8 & 14.5 & 153 & 95.7 & 0.19 & 0.34 & 0.90 & 0.47 & 0.43 & N \\ 
 139 & 5 34 53.1 & 5 45 49 & 61.8 & 3094 & 4.8 & 39.5 & 8.4 & 97 & 62.8 & 0.13 & 0.24 & 2.09 & 0.06 & 3.54 & N \\ 
 140 & 5 34 53.3 & 5 43 31 & 57.8 & 9056 & 6.1 & 42.6 & 15.5 & 53 & 107.4 & 0.22 & 0.44 & 6.16 & 0.13 & 2.08 & N \\ 
 141 & 5 34 53.6 & 4 56 60 & 88.5 & 4219 & 4.5 & 27.2 & 8.9 & 56 & 73.3 & 0.15 & 0.33 & 3.52 & 0.09 & 3.74 & N \\ 
 142 & 5 34 53.6 & 5 7 7 & 92.9 & 6806 & 2.3 & 24.0 & 16.9 & 121 & 93.1 & 0.19 & 0.46 & 1.53 & 0.48 & 0.79 & N \\ 
 143 & 5 34 53.7 & 5 11 30 & 86.5 & 4725 & 2.7 & 30.0 & 15.9 & 165 & 77.6 & 0.16 & 0.25 & 0.70 & 0.27 & 0.63 & N \\ 
 144 & 5 34 54.2 & 5 23 60 & 93.8 & 4275 & 2.7 & 31.8 & 9.4 & 70 & 73.8 & 0.15 & 0.48 & 1.23 & 0.52 & 1.28 & N \\ 
 145 & 5 34 54.2 & 5 31 52 & 56.7 & 6131 & 3.0 & 19.4 & 18.2 & 75 & 88.4 & 0.18 & 0.58 & 1.43 & 0.78 & 0.87 & N \\ 
 146 & 5 34 54.2 & 5 43 47 & 69.6 & 1688 & 5.1 & 17.6 & 7.1 & 135 & 46.4 & 0.09 & 0.26 & 0.88 & 0.13 & 3.68 & N \\ 
 147 & 5 34 54.4 & 6 20 47 & 54.8 & 6863 & 1.7 & 22.5 & 19.6 & -152 & 93.5 & 0.19 & 0.35 & 2.60 & 0.16 & 1.33 & N \\ 
 148 & 5 34 54.9 & 5 47 55 & 66.9 & 4275 & 3.3 & 31.9 & 10.3 & 103 & 73.8 & 0.15 & 0.37 & 1.12 & 0.35 & 1.17 & N \\ 
 149 & 5 34 56.2 & 5 35 7 & 68.1 & 3938 & 1.4 & 21.2 & 15.4 & 122 & 70.8 & 0.14 & 0.44 & 0.48 & 1.10 & 0.57 & N \\ 
 150 & 5 34 56.3 & 5 46 14 & 55.0 & 1125 & 3.5 & 9.0 & 7.8 & 85 & 37.8 & 0.08 & 0.20 & 1.09 & 0.05 & 8.37 & N \\ 
 151 & 5 34 56.4 & 5 42 16 & 68.9 & 6919 & 6.0 & 31.9 & 15.4 & 103 & 93.9 & 0.19 & 0.43 & 5.45 & 0.12 & 2.75 & N \\ 
 152 & 5 34 56.6 & 4 58 23 & 100.1 & 4275 & 1.3 & 22.6 & 14.5 & -138 & 73.8 & 0.15 & 0.21 & 0.42 & 0.29 & 0.44 & N \\ 
 153 & 5 34 56.6 & 5 41 59 & 52.6 & 9619 & 4.1 & 37.2 & 17.6 & 99 & 110.7 & 0.22 & 0.26 & 4.42 & 0.06 & 1.36 & N \\ 
 154 & 5 34 56.9 & 5 15 22 & 58.5 & 3375 & 1.5 & 19.7 & 16.5 & 148 & 65.6 & 0.13 & 0.45 & 0.32 & 1.56 & 0.48 & N \\ 
 155 & 5 34 56.9 & 6 21 43 & 44.0 & 2813 & 2.8 & 23.0 & 8.6 & 73 & 59.8 & 0.12 & 0.15 & 1.45 & 0.03 & 2.83 & N \\ 
 156 & 5 34 57.0 & 5 20 51 & 63.9 & 1350 & 4.6 & 12.3 & 6.6 & 61 & 41.5 & 0.08 & 0.25 & 0.69 & 0.15 & 4.07 & N \\ 
 157 & 5 34 57.0 & 5 44 11 & 49.7 & 6188 & 4.2 & 30.3 & 21.2 & -167 & 88.8 & 0.18 & 0.31 & 2.82 & 0.12 & 1.69 & N \\ 
 158 & 5 34 57.0 & 5 54 22 & 63.3 & 2813 & 4.3 & 18.6 & 10.5 & 174 & 59.8 & 0.12 & 0.30 & 1.04 & 0.19 & 2.03 & N \\ 
 159 & 5 34 57.7 & 5 49 49 & 61.6 & 3319 & 2.3 & 19.4 & 12.0 & 121 & 65.0 & 0.13 & 0.27 & 0.43 & 0.42 & 0.66 & N \\ 
 160 & 5 34 58.1 & 4 55 12 & 90.5 & 7200 & 5.1 & 41.9 & 18.4 & -178 & 95.7 & 0.19 & 0.25 & 3.37 & 0.07 & 1.60 & N \\ 
 161 & 5 34 58.1 & 5 6 28 & 89.1 & 3206 & 2.4 & 17.8 & 10.8 & 120 & 63.9 & 0.13 & 0.34 & 0.54 & 0.50 & 0.87 & N \\ 
 162 & 5 34 58.8 & 5 24 8 & 91.7 & 3038 & 2.4 & 20.6 & 11.2 & 120 & 62.2 & 0.12 & 0.16 & 0.80 & 0.08 & 1.39 & N \\ 
 163 & 5 34 58.8 & 6 23 9 & 44.7 & 3206 & 2.8 & 25.8 & 11.9 & 63 & 63.9 & 0.13 & 0.30 & 1.47 & 0.15 & 2.35 & N \\ 
 164 & 5 34 59.0 & 5 48 40 & 51.1 & 7650 & 5.2 & 33.1 & 14.4 & 91 & 98.7 & 0.20 & 0.32 & 4.84 & 0.08 & 2.10 & N \\ 
 165 & 5 34 59.0 & 6 16 59 & 43.4 & 3150 & 1.5 & 20.8 & 9.9 & 125 & 63.3 & 0.13 & 0.22 & 1.65 & 0.07 & 2.72 & N \\ 
 166 & 5 34 59.1 & 5 4 42 & 92.2 & 12881 & 2.5 & 51.8 & 22.0 & 118 & 128.1 & 0.26 & 0.43 & 2.31 & 0.39 & 0.46 & N \\ 
 167 & 5 34 59.3 & 4 58 19 & 88.5 & 3825 & 4.0 & 19.9 & 11.4 & -166 & 69.8 & 0.14 & 0.31 & 1.70 & 0.15 & 2.09 & N \\ 
 168 & 5 34 59.4 & 5 21 39 & 64.7 & 1069 & 4.6 & 8.7 & 6.7 & 46 & 36.9 & 0.07 & 0.61 & 1.88 & 0.27 & 15.62 & N \\ 
 169 & 5 34 59.5 & 5 53 34 & 54.3 & 3488 & 4.8 & 17.4 & 12.5 & 171 & 66.6 & 0.13 & 0.33 & 1.80 & 0.15 & 2.55 & N \\ 
 170 & 5 34 59.8 & 5 38 59 & 69.9 & 2925 & 5.2 & 21.4 & 9.0 & 134 & 61.0 & 0.12 & 0.20 & 2.25 & 0.04 & 4.14 & N \\ 
 171 & 5 34 59.8 & 5 48 32 & 74.3 & 3713 & 1.3 & 22.8 & 14.0 & -173 & 68.8 & 0.14 & 0.16 & 0.22 & 0.31 & 0.29 & N \\ 
 172 & 5 35 0.2 & 5 27 34 & 71.9 & 3150 & 1.6 & 16.5 & 10.8 & 161 & 63.3 & 0.13 & 0.46 & 0.69 & 0.72 & 1.14 & N \\ 
 173 & 5 35 0.2 & 5 50 4 & 49.0 & 2869 & 4.6 & 17.9 & 10.7 & 129 & 60.4 & 0.12 & 0.18 & 0.96 & 0.08 & 1.83 & N \\ 
 174 & 5 35 0.3 & 6 18 25 & 44.7 & 5231 & 2.5 & 24.5 & 13.1 & 156 & 81.6 & 0.16 & 0.32 & 2.94 & 0.11 & 2.26 & N \\ 
 175 & 5 35 0.4 & 5 50 16 & 66.9 & 2756 & 2.3 & 26.7 & 8.6 & 75 & 59.2 & 0.12 & 0.23 & 0.39 & 0.30 & 0.79 & N \\ 
 176 & 5 35 0.7 & 5 19 44 & 57.9 & 5006 & 2.4 & 17.6 & 16.0 & 73 & 79.8 & 0.16 & 0.76 & 2.20 & 0.80 & 1.80 & N \\ 
 177 & 5 35 0.8 & 5 2 17 & 107.2 & 4219 & 2.0 & 23.0 & 11.6 & 113 & 73.3 & 0.15 & 0.23 & 0.53 & 0.27 & 0.56 & N \\ 
 178 & 5 35 0.8 & 5 18 16 & 66.2 & 9338 & 3.0 & 22.8 & 22.2 & 178 & 109.0 & 0.22 & 0.75 & 3.86 & 0.61 & 1.24 & N \\ 
 179 & 5 35 0.8 & 5 59 54 & 78.8 & 1519 & 1.8 & 11.5 & 7.4 & -137 & 44.0 & 0.09 & 0.17 & 0.26 & 0.18 & 1.29 & N \\ 
 180 & 5 35 1.3 & 5 48 23 & 62.9 & 1800 & 2.1 & 19.5 & 7.1 & 135 & 47.9 & 0.10 & 0.20 & 0.23 & 0.30 & 0.88 & N \\ 
 181 & 5 35 1.3 & 6 20 15 & 63.5 & 3713 & 1.4 & 27.6 & 13.4 & 173 & 68.8 & 0.14 & 0.34 & 0.95 & 0.31 & 1.23 & N \\ 
 182 & 5 35 1.6 & 5 15 43 & 72.9 & 4669 & 4.3 & 25.3 & 11.6 & 111 & 77.1 & 0.15 & 0.55 & 2.42 & 0.36 & 2.21 & N \\ 
 183 & 5 35 1.7 & 5 13 44 & 78.3 & 4163 & 4.6 & 23.9 & 9.6 & 71 & 72.8 & 0.15 & 0.58 & 2.10 & 0.44 & 2.27 & N \\ 
 184 & 5 35 1.9 & 5 31 56 & 82.8 & 26381 & 1.7 & 67.2 & 29.4 & 64 & 183.3 & 0.37 & 0.58 & 9.18 & 0.25 & 0.62 & N \\ 
 185 & 5 35 1.9 & 6 15 32 & 39.8 & 3544 & 2.3 & 16.0 & 11.8 & 174 & 67.2 & 0.13 & 0.44 & 1.85 & 0.27 & 2.56 & N \\ 
 186 & 5 35 2.0 & 5 36 10 & 48.6 & 37350 & 7.6 & 67.3 & 36.4 & 114 & 218.1 & 0.44 & 0.74 & 44.44 & 0.10 & 1.79 & Y \\ 
 187 & 5 35 2.2 & 5 1 35 & 93.2 & 9956 & 3.8 & 28.4 & 23.0 & -140 & 112.6 & 0.23 & 0.36 & 2.32 & 0.24 & 0.68 & N \\ 
 188 & 5 35 2.2 & 5 55 19 & 61.3 & 8888 & 5.3 & 43.0 & 15.0 & 55 & 106.4 & 0.21 & 0.50 & 7.43 & 0.14 & 2.58 & N \\ 
 189 & 5 35 2.3 & 5 32 10 & 62.5 & 2250 & 1.6 & 18.9 & 8.4 & 115 & 53.5 & 0.11 & 0.24 & 0.37 & 0.32 & 1.02 & N \\ 
 190 & 5 35 2.7 & 5 46 39 & 79.6 & 17663 & 1.6 & 61.2 & 20.5 & 103 & 150.0 & 0.30 & 0.54 & 4.09 & 0.40 & 0.51 & N \\ 
 191 & 5 35 2.9 & 5 2 35 & 101.9 & 6075 & 2.2 & 29.9 & 18.5 & 132 & 87.9 & 0.18 & 0.36 & 0.58 & 0.74 & 0.36 & N \\ 
 192 & 5 35 3.1 & 4 53 52 & 39.9 & 1856 & 1.6 & 14.1 & 10.5 & -152 & 48.6 & 0.10 & 0.22 & 0.17 & 0.51 & 0.61 & N \\ 
 193 & 5 35 3.1 & 5 0 48 & 101.6 & 8325 & 2.7 & 28.5 & 17.4 & 162 & 103.0 & 0.21 & 0.36 & 1.44 & 0.35 & 0.55 & N \\ 
 194 & 5 35 3.2 & 5 23 36 & 83.6 & 2250 & 2.0 & 15.7 & 8.6 & -140 & 53.5 & 0.11 & 0.41 & 0.72 & 0.47 & 1.97 & N \\ 
 195 & 5 35 3.6 & 4 52 13 & 104.0 & 4331 & 2.3 & 25.0 & 17.5 & 99 & 74.3 & 0.15 & 0.22 & 0.21 & 0.67 & 0.22 & N \\ 
 196 & 5 35 3.6 & 5 25 58 & 95.9 & 11644 & 2.6 & 40.4 & 20.8 & -149 & 121.8 & 0.24 & 0.82 & 3.95 & 0.79 & 0.91 & N \\ 
 197 & 5 35 4.2 & 5 39 22 & 56.4 & 4163 & 3.3 & 20.5 & 13.0 & 142 & 72.8 & 0.15 & 0.30 & 1.09 & 0.23 & 1.18 & N \\ 
 198 & 5 35 4.3 & 5 24 29 & 66.8 & 7200 & 2.5 & 39.4 & 10.8 & 149 & 95.7 & 0.19 & 0.93 & 4.46 & 0.71 & 2.12 & N \\ 
 199 & 5 35 4.4 & 5 37 41 & 65.7 & 2194 & 5.3 & 21.3 & 7.6 & 127 & 52.9 & 0.11 & 0.27 & 2.05 & 0.07 & 5.82 & Y \\ 
 200 & 5 35 4.6 & 4 57 43 & 93.9 & 2813 & 5.0 & 16.9 & 10.5 & -146 & 59.8 & 0.12 & 0.27 & 1.49 & 0.11 & 2.91 & N \\ 
 201 & 5 35 4.6 & 5 7 36 & 87.3 & 4725 & 2.2 & 25.4 & 13.0 & 88 & 77.6 & 0.16 & 0.30 & 0.35 & 0.77 & 0.31 & N \\ 
 202 & 5 35 4.6 & 5 22 59 & 65.3 & 3938 & 2.3 & 16.3 & 13.8 & -135 & 70.8 & 0.14 & 0.62 & 1.50 & 0.70 & 1.77 & N \\ 
 203 & 5 35 4.6 & 6 19 27 & 70.2 & 8550 & 1.6 & 29.8 & 21.2 & 135 & 104.3 & 0.21 & 0.57 & 2.55 & 0.50 & 0.94 & N \\ 
 204 & 5 35 4.7 & 4 59 25 & 85.3 & 4669 & 2.9 & 28.3 & 18.4 & -146 & 77.1 & 0.15 & 0.41 & 0.76 & 0.66 & 0.69 & N \\ 
 205 & 5 35 4.8 & 4 50 49 & 57.0 & 3319 & 1.9 & 18.5 & 12.7 & 63 & 65.0 & 0.13 & 0.31 & 0.12 & 1.91 & 0.18 & N \\ 
 206 & 5 35 5.2 & 5 3 50 & 95.3 & 5681 & 2.7 & 24.8 & 20.1 & -147 & 85.1 & 0.17 & 0.20 & 0.50 & 0.25 & 0.34 & N \\ 
 207 & 5 35 5.2 & 6 11 29 & 59.8 & 8213 & 3.4 & 29.3 & 19.6 & 110 & 102.3 & 0.21 & 0.28 & 3.97 & 0.08 & 1.55 & N \\ 
 208 & 5 35 5.2 & 6 16 13 & 41.2 & 3038 & 2.0 & 14.3 & 13.1 & 126 & 62.2 & 0.12 & 0.26 & 1.58 & 0.10 & 2.75 & N \\ 
 209 & 5 35 5.3 & 6 13 12 & 63.1 & 5175 & 2.9 & 32.0 & 18.6 & -151 & 81.2 & 0.16 & 0.16 & 1.62 & 0.05 & 1.27 & N \\ 
 210 & 5 35 5.4 & 6 19 19 & 40.7 & 4331 & 2.1 & 20.9 & 12.1 & 79 & 74.3 & 0.15 & 0.35 & 1.37 & 0.25 & 1.40 & N \\ 
 211 & 5 35 5.5 & 5 13 40 & 73.9 & 2475 & 3.8 & 16.2 & 8.8 & 70 & 56.1 & 0.11 & 0.28 & 0.55 & 0.31 & 1.30 & N \\ 
 212 & 5 35 6.0 & 5 31 11 & 102.4 & 9338 & 1.6 & 26.2 & 22.5 & -171 & 109.0 & 0.22 & 0.51 & 3.63 & 0.30 & 1.17 & N \\ 
 213 & 5 35 6.1 & 5 22 52 & 48.3 & 2081 & 2.7 & 13.4 & 8.2 & -147 & 51.5 & 0.10 & 0.52 & 1.42 & 0.37 & 4.36 & N \\ 
 214 & 5 35 6.3 & 5 43 12 & 63.0 & 2869 & 2.5 & 19.1 & 10.1 & 81 & 60.4 & 0.12 & 0.18 & 0.74 & 0.10 & 1.40 & N \\ 
 215 & 5 35 6.3 & 6 2 53 & 70.1 & 7819 & 2.8 & 27.0 & 18.9 & 66 & 99.8 & 0.20 & 0.36 & 2.87 & 0.17 & 1.21 & N \\ 
 216 & 5 35 6.3 & 6 21 58 & 65.8 & 11025 & 1.5 & 41.8 & 23.8 & 110 & 118.5 & 0.24 & 0.50 & 3.96 & 0.28 & 0.99 & N \\ 
 217 & 5 35 6.6 & 4 55 8 & 111.7 & 3263 & 2.3 & 20.1 & 11.8 & 88 & 64.5 & 0.13 & 0.21 & 0.41 & 0.27 & 0.64 & N \\ 
 218 & 5 35 6.9 & 4 54 34 & 36.5 & 2419 & 2.4 & 19.5 & 8.2 & 67 & 55.5 & 0.11 & 0.34 & 0.32 & 0.75 & 0.79 & N \\ 
 219 & 5 35 6.9 & 5 30 5 & 70.1 & 4444 & 1.6 & 19.5 & 13.1 & -163 & 75.2 & 0.15 & 0.50 & 1.26 & 0.57 & 1.23 & N \\ 
 220 & 5 35 7.4 & 5 58 22 & 62.2 & 26663 & 5.6 & 60.0 & 27.6 & 70 & 184.2 & 0.37 & 0.47 & 22.07 & 0.07 & 1.47 & Y \\ 
 221 & 5 35 7.6 & 5 15 27 & 75.1 & 10688 & 4.2 & 34.3 & 22.5 & -171 & 116.7 & 0.23 & 0.46 & 2.80 & 0.34 & 0.74 & N \\ 
 222 & 5 35 7.9 & 5 12 14 & 60.2 & 7763 & 1.7 & 27.5 & 15.4 & 93 & 99.4 & 0.20 & 0.54 & 0.90 & 1.23 & 0.38 & N \\ 
 223 & 5 35 8.1 & 5 0 55 & 92.0 & 1463 & 2.9 & 14.1 & 7.4 & 51 & 43.2 & 0.09 & 0.19 & 0.14 & 0.42 & 0.74 & N \\ 
 224 & 5 35 8.1 & 5 51 28 & 46.9 & 2700 & 3.6 & 14.7 & 12.7 & 64 & 58.6 & 0.12 & 0.26 & 2.59 & 0.06 & 5.37 & N \\ 
 225 & 5 35 8.6 & 4 59 25 & 82.0 & 3319 & 3.8 & 25.8 & 10.4 & 170 & 65.0 & 0.13 & 0.23 & 0.39 & 0.34 & 0.60 & N \\ 
 226 & 5 35 8.6 & 6 5 55 & 54.2 & 4219 & 3.3 & 17.9 & 13.3 & 64 & 73.3 & 0.15 & 0.39 & 2.36 & 0.18 & 2.50 & N \\ 
 227 & 5 35 8.6 & 6 17 13 & 43.3 & 5794 & 2.2 & 32.8 & 13.7 & 66 & 85.9 & 0.17 & 0.40 & 1.97 & 0.26 & 1.30 & N \\ 
 228 & 5 35 8.7 & 6 3 56 & 75.4 & 6075 & 2.0 & 24.5 & 15.2 & 122 & 87.9 & 0.18 & 0.36 & 1.34 & 0.32 & 0.82 & N \\ 
 229 & 5 35 9.0 & 6 11 43 & 53.4 & 4556 & 3.1 & 31.7 & 12.7 & -156 & 76.2 & 0.15 & 0.40 & 1.54 & 0.30 & 1.45 & N \\ 
 230 & 5 35 9.3 & 6 4 1 & 61.6 & 9956 & 3.7 & 27.5 & 19.6 & 63 & 112.6 & 0.23 & 0.63 & 4.80 & 0.35 & 1.41 & N \\ 
 231 & 5 35 9.7 & 5 35 15 & 59.1 & 10575 & 6.3 & 51.4 & 12.6 & 123 & 116.0 & 0.23 & 0.52 & 14.80 & 0.08 & 3.96 & Y \\ 
 232 & 5 35 10.0 & 5 1 20 & 35.1 & 2475 & 3.0 & 16.1 & 10.8 & 155 & 56.1 & 0.11 & 0.20 & 0.16 & 0.54 & 0.37 & N \\ 
 233 & 5 35 10.0 & 5 17 24 & 71.4 & 7425 & 4.7 & 24.6 & 17.1 & 83 & 97.2 & 0.20 & 0.45 & 4.19 & 0.18 & 1.91 & N \\ 
 234 & 5 35 10.4 & 5 38 13 & 53.2 & 6244 & 4.1 & 21.9 & 14.6 & 78 & 89.2 & 0.18 & 0.77 & 4.58 & 0.44 & 2.70 & N \\ 
 235 & 5 35 10.5 & 5 2 47 & 98.3 & 2194 & 2.6 & 27.6 & 7.5 & -174 & 52.9 & 0.11 & 0.31 & 0.13 & 1.47 & 0.38 & N \\ 
 236 & 5 35 10.5 & 5 32 31 & 37.6 & 3938 & 2.9 & 18.0 & 13.1 & 74 & 70.8 & 0.14 & 0.45 & 1.68 & 0.32 & 1.97 & N \\ 
 237 & 5 35 10.7 & 5 29 8 & 90.2 & 3150 & 3.4 & 15.4 & 11.2 & 134 & 63.3 & 0.13 & 0.45 & 1.55 & 0.31 & 2.55 & N \\ 
 238 & 5 35 10.9 & 6 14 34 & 37.1 & 28631 & 3.7 & 43.7 & 35.3 & 80 & 190.9 & 0.38 & 0.67 & 36.42 & 0.09 & 2.19 & N \\ 
 239 & 5 35 11.1 & 5 8 29 & 88.8 & 4500 & 4.5 & 21.2 & 14.5 & 120 & 75.7 & 0.15 & 0.44 & 0.67 & 0.83 & 0.65 & N \\ 
 240 & 5 35 11.2 & 4 53 30 & 89.6 & 3769 & 3.1 & 27.1 & 12.2 & -148 & 69.3 & 0.14 & 0.16 & 0.15 & 0.47 & 0.18 & N \\ 
 241 & 5 35 11.4 & 4 50 51 & 57.0 & 6300 & 2.5 & 33.9 & 15.2 & -160 & 89.6 & 0.18 & 0.43 & 0.06 & 9.72 & 0.04 & N \\ 
 242 & 5 35 11.7 & 5 6 35 & 92.0 & 2644 & 3.4 & 23.4 & 8.7 & 91 & 58.0 & 0.12 & 0.27 & 0.24 & 0.66 & 0.51 & N \\ 
 243 & 5 35 11.7 & 5 59 34 & 73.0 & 3094 & 4.1 & 17.2 & 12.1 & 121 & 62.8 & 0.13 & 0.25 & 1.30 & 0.11 & 2.20 & N \\ 
 244 & 5 35 11.9 & 4 59 59 & 43.5 & 4781 & 3.5 & 23.9 & 16.4 & -144 & 78.0 & 0.16 & 0.25 & 0.48 & 0.38 & 0.42 & Y \\ 
 245 & 5 35 11.9 & 5 52 37 & 58.7 & 9281 & 2.8 & 37.1 & 15.3 & -151 & 108.7 & 0.22 & 0.41 & 5.08 & 0.14 & 1.65 & Y \\ 
 246 & 5 35 11.9 & 6 11 1 & 49.7 & 3150 & 2.7 & 25.0 & 11.9 & 137 & 63.3 & 0.13 & 0.31 & 0.77 & 0.30 & 1.27 & N \\ 
 247 & 5 35 12.4 & 5 28 15 & 80.0 & 2925 & 3.0 & 19.5 & 11.5 & 123 & 61.0 & 0.12 & 0.38 & 0.93 & 0.36 & 1.72 & N \\ 
 248 & 5 35 12.5 & 4 58 47 & 88.6 & 4838 & 8.4 & 31.7 & 10.7 & 57 & 78.5 & 0.16 & 0.51 & 5.25 & 0.15 & 4.53 & N \\ 
 249 & 5 35 12.6 & 6 8 29 & 48.3 & 5456 & 1.4 & 28.1 & 16.5 & 88 & 83.3 & 0.17 & 0.24 & 0.93 & 0.19 & 0.67 & N \\ 
 250 & 5 35 12.7 & 5 8 7 & 112.8 & 6525 & 3.0 & 29.2 & 21.1 & 98 & 91.1 & 0.18 & 0.31 & 0.29 & 1.14 & 0.16 & N \\ 
 251 & 5 35 12.9 & 5 12 49 & 66.6 & 5231 & 2.0 & 19.5 & 11.8 & 94 & 81.6 & 0.16 & 0.71 & 0.68 & 2.26 & 0.53 & N \\ 
 252 & 5 35 13.2 & 5 23 58 & 50.9 & 1913 & 4.6 & 16.6 & 6.7 & 102 & 49.3 & 0.10 & 0.46 & 6.46 & 0.06 & 22.46 & N \\ 
 253 & 5 35 13.2 & 6 19 13 & 45.6 & 5175 & 2.2 & 27.1 & 13.4 & 115 & 81.2 & 0.16 & 0.26 & 1.92 & 0.11 & 1.50 & N \\ 
 254 & 5 35 13.3 & 4 54 10 & 57.0 & 1463 & 1.9 & 14.5 & 6.7 & 159 & 43.2 & 0.09 & 0.20 & 0.08 & 0.79 & 0.42 & N \\ 
 255 & 5 35 13.3 & 5 26 37 & 66.3 & 2194 & 5.4 & 14.6 & 8.9 & 119 & 52.9 & 0.11 & 0.62 & 3.51 & 0.22 & 9.94 & N \\ 
 256 & 5 35 13.4 & 5 23 7 & 63.7 & 2138 & 5.1 & 14.1 & 7.9 & 95 & 52.2 & 0.10 & 0.82 & 13.51 & 0.10 & 39.76 & N \\ 
 257 & 5 35 13.4 & 5 24 2 & 41.0 & 1013 & 5.3 & 8.8 & 5.9 & 93 & 35.9 & 0.07 & 0.76 & 8.28 & 0.09 & 74.72 & N \\ 
 258 & 5 35 13.9 & 6 1 9 & 74.5 & 7875 & 4.6 & 29.7 & 15.4 & 80 & 100.1 & 0.20 & 0.23 & 2.99 & 0.07 & 1.25 & N \\ 
 259 & 5 35 14.0 & 5 0 10 & 67.7 & 6019 & 2.7 & 28.4 & 19.7 & 130 & 87.5 & 0.18 & 0.32 & 0.77 & 0.43 & 0.48 & Y \\ 
 260 & 5 35 14.0 & 6 9 5 & 69.1 & 5681 & 1.5 & 32.6 & 12.5 & 163 & 85.1 & 0.17 & 0.24 & 1.39 & 0.13 & 0.95 & N \\ 
 261 & 5 35 14.0 & 6 12 18 & 66.1 & 2081 & 1.6 & 18.4 & 8.4 & 143 & 51.5 & 0.10 & 0.19 & 0.25 & 0.30 & 0.75 & N \\ 
 262 & 5 35 14.1 & 6 13 0 & 48.8 & 6638 & 4.0 & 24.5 & 19.7 & -160 & 91.9 & 0.18 & 0.21 & 3.81 & 0.04 & 2.05 & N \\ 
 263 & 5 35 14.5 & 5 37 33 & 66.4 & 4669 & 2.0 & 24.5 & 13.0 & 112 & 77.1 & 0.15 & 0.55 & 0.82 & 1.06 & 0.75 & N \\ 
 264 & 5 35 14.7 & 5 58 30 & 55.4 & 2644 & 4.5 & 16.0 & 10.4 & -145 & 58.0 & 0.12 & 0.24 & 1.87 & 0.07 & 4.00 & N \\ 
 265 & 5 35 14.9 & 5 4 48 & 89.3 & 2981 & 4.9 & 20.2 & 10.9 & 56 & 61.6 & 0.12 & 0.32 & 0.60 & 0.39 & 1.07 & N \\ 
 266 & 5 35 14.9 & 5 9 30 & 74.8 & 2644 & 1.9 & 17.8 & 9.8 & 116 & 58.0 & 0.12 & 0.37 & 0.33 & 0.90 & 0.70 & N \\ 
 267 & 5 35 15.1 & 6 17 1 & 47.2 & 8044 & 2.3 & 31.3 & 19.9 & 86 & 101.2 & 0.20 & 0.41 & 3.76 & 0.17 & 1.52 & N \\ 
 268 & 5 35 15.4 & 5 4 43 & 84.6 & 3431 & 5.4 & 17.2 & 13.5 & 94 & 66.1 & 0.13 & 0.37 & 0.89 & 0.39 & 1.29 & N \\ 
 269 & 5 35 15.5 & 5 11 47 & 86.7 & 5288 & 5.0 & 27.2 & 11.7 & 77 & 82.1 & 0.16 & 0.50 & 4.80 & 0.17 & 3.63 & N \\ 
 270 & 5 35 15.5 & 5 15 41 & 82.0 & 6131 & 3.7 & 38.5 & 10.7 & 95 & 88.4 & 0.18 & 0.39 & 3.44 & 0.15 & 2.08 & N \\ 
 271 & 5 35 15.8 & 5 0 21 & 83.0 & 2194 & 7.1 & 13.4 & 9.4 & 175 & 52.9 & 0.11 & 0.39 & 2.15 & 0.14 & 6.10 & Y \\ 
 272 & 5 35 15.8 & 5 59 52 & 58.4 & 7763 & 4.1 & 33.0 & 17.7 & 136 & 99.4 & 0.20 & 0.33 & 3.00 & 0.14 & 1.28 & N \\ 
 273 & 5 35 15.9 & 5 3 18 & 83.7 & 3206 & 5.6 & 29.3 & 10.2 & 110 & 63.9 & 0.13 & 0.29 & 0.76 & 0.27 & 1.22 & N \\ 
 274 & 5 35 16.0 & 5 21 39 & 79.4 & 5231 & 6.9 & 30.3 & 10.2 & 101 & 81.6 & 0.16 & 0.80 & 48.90 & 0.04 & 37.58 & N \\ 
 275 & 5 35 16.4 & 5 13 31 & 84.5 & 3150 & 4.3 & 24.7 & 8.2 & 71 & 63.3 & 0.13 & 0.33 & 1.83 & 0.14 & 3.01 & N \\ 
 276 & 5 35 16.4 & 5 26 16 & 77.1 & 2250 & 5.2 & 17.8 & 7.3 & 123 & 53.5 & 0.11 & 0.53 & 2.79 & 0.21 & 7.59 & N \\ 
 277 & 5 35 16.5 & 5 30 44 & 40.9 & 12150 & 4.7 & 37.0 & 16.4 & 113 & 124.4 & 0.25 & 0.62 & 9.84 & 0.18 & 2.14 & N \\ 
 278 & 5 35 16.9 & 6 5 27 & 50.9 & 9225 & 2.3 & 34.3 & 21.5 & 92 & 108.4 & 0.22 & 0.31 & 1.71 & 0.23 & 0.56 & N \\ 
 279 & 5 35 17.1 & 5 19 26 & 72.8 & 1856 & 5.5 & 14.5 & 7.5 & 133 & 48.6 & 0.10 & 0.32 & 7.20 & 0.03 & 26.19 & N \\ 
 280 & 5 35 17.2 & 6 38 36 & 64.4 & 7763 & 1.5 & 36.5 & 23.4 & 136 & 99.4 & 0.20 & 0.22 & 2.23 & 0.08 & 0.95 & N \\ 
 281 & 5 35 17.3 & 5 58 25 & 80.8 & 11475 & 1.9 & 40.7 & 23.7 & 62 & 120.9 & 0.24 & 0.26 & 1.51 & 0.21 & 0.36 & Y \\ 
 282 & 5 35 17.8 & 6 3 21 & 73.1 & 4444 & 2.7 & 19.2 & 15.9 & 129 & 75.2 & 0.15 & 0.22 & 0.72 & 0.19 & 0.70 & N \\ 
 283 & 5 35 17.9 & 6 15 54 & 41.3 & 2363 & 1.6 & 18.3 & 9.2 & 100 & 54.8 & 0.11 & 0.29 & 0.95 & 0.19 & 2.41 & N \\ 
 284 & 5 35 18.0 & 5 1 39 & 84.0 & 1519 & 5.8 & 12.8 & 6.6 & 87 & 44.0 & 0.09 & 0.28 & 1.74 & 0.08 & 8.53 & N \\ 
 285 & 5 35 18.3 & 5 9 19 & 89.3 & 4781 & 5.4 & 29.2 & 12.5 & 86 & 78.0 & 0.16 & 0.32 & 2.91 & 0.10 & 2.56 & N \\ 
 286 & 5 35 18.4 & 5 0 31 & 90.8 & 5175 & 7.8 & 30.2 & 13.0 & -164 & 81.2 & 0.16 & 0.31 & 16.72 & 0.02 & 13.06 & Y \\ 
 287 & 5 35 19.2 & 5 4 52 & 72.7 & 1800 & 3.3 & 14.8 & 7.3 & 55 & 47.9 & 0.10 & 0.34 & 0.86 & 0.25 & 3.29 & N \\ 
 288 & 5 35 19.6 & 5 18 27 & 74.1 & 1575 & 5.3 & 12.7 & 6.8 & 113 & 44.8 & 0.09 & 0.48 & 4.48 & 0.09 & 20.82 & N \\ 
 289 & 5 35 19.6 & 6 20 31 & 46.3 & 15863 & 2.9 & 42.2 & 26.1 & 71 & 142.1 & 0.29 & 0.31 & 7.03 & 0.08 & 1.02 & N \\ 
 290 & 5 35 19.6 & 6 34 28 & 68.7 & 13050 & 2.8 & 37.2 & 23.8 & 95 & 128.9 & 0.26 & 0.29 & 2.91 & 0.14 & 0.57 & N \\ 
 291 & 5 35 19.8 & 5 16 59 & 90.3 & 2081 & 2.3 & 16.6 & 9.1 & 145 & 51.5 & 0.10 & 0.20 & 0.40 & 0.20 & 1.23 & N \\ 
 292 & 5 35 20.0 & 4 56 45 & 100.1 & 3150 & 3.8 & 22.1 & 9.4 & -162 & 63.3 & 0.13 & 0.46 & 1.06 & 0.48 & 1.74 & N \\ 
 293 & 5 35 20.4 & 6 8 27 & 67.2 & 6188 & 1.7 & 35.8 & 17.4 & 168 & 88.8 & 0.18 & 0.35 & 1.07 & 0.38 & 0.64 & N \\ 
 294 & 5 35 20.6 & 5 38 52 & 72.8 & 4050 & 1.4 & 30.6 & 13.0 & 117 & 71.8 & 0.14 & 0.37 & 1.51 & 0.24 & 1.70 & N \\ 
 295 & 5 35 20.6 & 6 7 16 & 64.7 & 3544 & 1.8 & 28.4 & 12.0 & 124 & 67.2 & 0.13 & 0.17 & 0.41 & 0.18 & 0.57 & N \\ 
 296 & 5 35 21.1 & 6 23 1 & 68.4 & 9900 & 1.5 & 70.8 & 24.6 & 95 & 112.3 & 0.23 & 0.33 & 1.76 & 0.27 & 0.52 & N \\ 
 297 & 5 35 21.4 & 5 55 46 & 59.2 & 1406 & 1.6 & 13.6 & 7.4 & 102 & 42.3 & 0.08 & 0.23 & 0.40 & 0.22 & 2.20 & N \\ 
 298 & 5 35 21.5 & 6 13 8 & 33.8 & 1406 & 2.2 & 11.7 & 7.0 & 169 & 42.3 & 0.08 & 0.26 & 1.10 & 0.10 & 6.06 & Y \\ 
 299 & 5 35 21.7 & 5 6 17 & 88.9 & 6525 & 5.4 & 24.2 & 16.8 & 95 & 91.1 & 0.18 & 0.45 & 6.66 & 0.10 & 3.68 & N \\ 
 300 & 5 35 21.7 & 5 8 5 & 88.3 & 4106 & 5.6 & 28.1 & 9.0 & 68 & 72.3 & 0.15 & 0.49 & 4.15 & 0.16 & 4.58 & N \\ 
 301 & 5 35 21.8 & 6 3 24 & 61.8 & 12094 & 5.2 & 35.3 & 20.4 & 89 & 124.1 & 0.25 & 0.60 & 8.17 & 0.21 & 1.79 & N \\ 
 302 & 5 35 21.8 & 6 7 45 & 77.7 & 3825 & 1.7 & 23.2 & 13.5 & 60 & 69.8 & 0.14 & 0.33 & 0.54 & 0.54 & 0.67 & N \\ 
 303 & 5 35 22.0 & 6 8 27 & 55.3 & 4219 & 1.6 & 24.5 & 16.1 & 46 & 73.3 & 0.15 & 0.32 & 0.42 & 0.70 & 0.44 & N \\ 
 304 & 5 35 22.3 & 6 13 30 & 39.2 & 3319 & 2.0 & 26.5 & 10.9 & 162 & 65.0 & 0.13 & 0.37 & 1.63 & 0.21 & 2.47 & Y \\ 
 305 & 5 35 22.4 & 6 7 58 & 82.9 & 1688 & 1.7 & 24.9 & 6.1 & 79 & 46.4 & 0.09 & 0.26 & 0.13 & 0.91 & 0.55 & N \\ 
 306 & 5 35 22.5 & 5 14 48 & 84.3 & 4669 & 4.0 & 23.8 & 13.8 & 98 & 77.1 & 0.15 & 0.36 & 3.91 & 0.10 & 3.57 & N \\ 
 307 & 5 35 22.5 & 5 25 19 & 83.6 & 1856 & 2.9 & 13.3 & 7.5 & 149 & 48.6 & 0.10 & 0.40 & 1.29 & 0.23 & 4.70 & N \\ 
 308 & 5 35 22.5 & 6 1 36 & 27.0 & 2194 & 1.6 & 18.2 & 8.6 & 135 & 52.9 & 0.11 & 0.15 & 0.12 & 0.38 & 0.35 & N \\ 
 309 & 5 35 22.7 & 5 20 20 & 93.6 & 2419 & 1.5 & 17.5 & 8.8 & 57 & 55.5 & 0.11 & 0.28 & 0.75 & 0.22 & 1.85 & N \\ 
 310 & 5 35 23.0 & 5 54 51 & 67.3 & 3038 & 3.5 & 14.8 & 11.5 & 101 & 62.2 & 0.12 & 0.26 & 1.07 & 0.15 & 1.86 & N \\ 
 311 & 5 35 23.7 & 5 36 6 & 70.3 & 3825 & 1.7 & 19.0 & 14.1 & 116 & 69.8 & 0.14 & 0.36 & 0.96 & 0.36 & 1.18 & N \\ 
 312 & 5 35 23.9 & 5 56 39 & 57.1 & 3263 & 1.9 & 19.6 & 12.0 & -148 & 64.5 & 0.13 & 0.24 & 0.53 & 0.26 & 0.82 & N \\ 
 313 & 5 35 24.0 & 5 13 9 & 85.1 & 3713 & 3.5 & 20.9 & 14.1 & 128 & 68.8 & 0.14 & 0.24 & 3.69 & 0.04 & 4.74 & Y \\ 
 314 & 5 35 24.0 & 5 22 33 & 84.2 & 4669 & 1.4 & 27.7 & 15.0 & -162 & 77.1 & 0.15 & 0.33 & 1.77 & 0.18 & 1.61 & N \\ 
 315 & 5 35 24.1 & 5 25 13 & 59.6 & 3656 & 1.4 & 26.6 & 13.8 & -144 & 68.2 & 0.14 & 0.19 & 0.38 & 0.25 & 0.50 & N \\ 
 316 & 5 35 24.4 & 6 19 2 & 41.4 & 2475 & 1.9 & 15.2 & 10.4 & -165 & 56.1 & 0.11 & 0.32 & 0.82 & 0.26 & 1.93 & N \\ 
 317 & 5 35 24.5 & 5 59 28 & 52.4 & 6694 & 3.3 & 30.1 & 14.5 & 148 & 92.3 & 0.19 & 0.36 & 3.16 & 0.15 & 1.68 & N \\ 
 318 & 5 35 24.6 & 4 53 9 & 92.3 & 2700 & 1.5 & 20.5 & 9.4 & -157 & 58.6 & 0.12 & 0.19 & 0.51 & 0.16 & 1.05 & N \\ 
 319 & 5 35 25.5 & 5 55 10 & 73.9 & 1969 & 1.7 & 14.2 & 9.8 & 142 & 50.1 & 0.10 & 0.24 & 0.26 & 0.41 & 0.87 & N \\ 
 320 & 5 35 25.5 & 6 40 9 & 60.7 & 7256 & 2.7 & 27.9 & 13.2 & 126 & 96.1 & 0.19 & 0.40 & 2.31 & 0.26 & 1.09 & N \\ 
 321 & 5 35 25.6 & 6 0 47 & 33.8 & 18956 & 2.2 & 42.6 & 27.4 & 108 & 155.4 & 0.31 & 0.41 & 3.46 & 0.29 & 0.39 & N \\ 
 322 & 5 35 25.7 & 5 2 40 & 90.1 & 1463 & 4.9 & 15.3 & 7.3 & 78 & 43.2 & 0.09 & 0.28 & 2.50 & 0.05 & 12.99 & N \\ 
 323 & 5 35 25.8 & 5 20 18 & 42.9 & 2419 & 2.2 & 16.6 & 8.2 & -160 & 55.5 & 0.11 & 0.48 & 1.34 & 0.36 & 3.28 & N \\ 
 324 & 5 35 25.9 & 5 51 45 & 57.3 & 18563 & 6.2 & 44.6 & 25.8 & 62 & 153.7 & 0.31 & 0.55 & 14.70 & 0.12 & 1.69 & N \\ 
 325 & 5 35 25.9 & 5 53 21 & 51.1 & 2250 & 3.7 & 22.3 & 8.3 & -159 & 53.5 & 0.11 & 0.21 & 0.98 & 0.09 & 2.68 & N \\ 
 326 & 5 35 26.3 & 5 20 19 & 49.1 & 1519 & 2.2 & 10.4 & 8.8 & -167 & 44.0 & 0.09 & 0.20 & 0.76 & 0.09 & 3.74 & N \\ 
 327 & 5 35 26.3 & 5 55 13 & 41.3 & 7481 & 2.5 & 27.7 & 15.8 & 120 & 97.6 & 0.20 & 0.45 & 2.54 & 0.29 & 1.14 & N \\ 
 328 & 5 35 26.5 & 6 0 41 & 45.9 & 12938 & 2.8 & 38.9 & 24.1 & 147 & 128.3 & 0.26 & 0.38 & 3.34 & 0.21 & 0.66 & N \\ 
 329 & 5 35 26.6 & 5 50 55 & 50.2 & 2644 & 1.5 & 18.5 & 11.0 & 178 & 58.0 & 0.12 & 0.21 & 0.16 & 0.59 & 0.34 & N \\ 
 330 & 5 35 26.9 & 6 41 19 & 61.6 & 5175 & 1.9 & 20.9 & 15.9 & 129 & 81.2 & 0.16 & 0.29 & 1.37 & 0.18 & 1.07 & N \\ 
 331 & 5 35 27.0 & 5 24 39 & 82.4 & 6694 & 3.1 & 34.9 & 12.8 & 168 & 92.3 & 0.19 & 0.86 & 3.98 & 0.65 & 2.11 & N \\ 
 332 & 5 35 27.4 & 5 14 20 & 96.2 & 4669 & 1.4 & 32.1 & 20.3 & 150 & 77.1 & 0.15 & 0.17 & 0.42 & 0.19 & 0.39 & N \\ 
 333 & 5 35 27.6 & 6 38 14 & 63.6 & 2869 & 2.5 & 18.8 & 10.4 & 111 & 60.4 & 0.12 & 0.22 & 0.60 & 0.18 & 1.13 & N \\ 
 334 & 5 35 27.8 & 5 5 43 & 93.9 & 4725 & 6.2 & 25.8 & 13.8 & 130 & 77.6 & 0.16 & 0.29 & 9.78 & 0.02 & 8.76 & Y \\ 
 335 & 5 35 27.8 & 6 21 31 & 45.1 & 2531 & 1.4 & 19.6 & 12.1 & 96 & 56.8 & 0.11 & 0.19 & 1.27 & 0.06 & 2.90 & N \\ 
 336 & 5 35 28.3 & 5 36 29 & 72.1 & 2588 & 1.5 & 19.4 & 9.4 & 61 & 57.4 & 0.12 & 0.24 & 1.00 & 0.13 & 2.21 & N \\ 
 337 & 5 35 28.5 & 6 5 44 & 63.8 & 4106 & 3.6 & 23.9 & 11.5 & 167 & 72.3 & 0.15 & 0.38 & 1.75 & 0.22 & 1.93 & N \\ 
 338 & 5 35 28.6 & 6 30 12 & 67.3 & 3319 & 4.7 & 20.6 & 10.9 & 92 & 65.0 & 0.13 & 0.20 & 1.50 & 0.07 & 2.28 & N \\ 
 339 & 5 35 28.7 & 5 7 29 & 93.6 & 3544 & 4.6 & 20.8 & 12.7 & 151 & 67.2 & 0.13 & 0.26 & 3.12 & 0.06 & 4.30 & Y \\ 
 340 & 5 35 29.3 & 4 58 20 & 97.0 & 6919 & 7.6 & 31.6 & 14.0 & 67 & 93.9 & 0.19 & 0.59 & 11.18 & 0.11 & 5.65 & Y \\ 
 341 & 5 35 29.3 & 5 22 57 & 68.8 & 4388 & 1.6 & 25.9 & 13.2 & 56 & 74.7 & 0.15 & 0.20 & 1.72 & 0.07 & 1.72 & N \\ 
 342 & 5 35 29.3 & 5 39 6 & 78.8 & 6975 & 1.4 & 35.4 & 18.3 & 147 & 94.2 & 0.19 & 0.18 & 2.33 & 0.05 & 1.16 & N \\ 
 343 & 5 35 29.5 & 5 53 39 & 44.1 & 2588 & 2.9 & 13.2 & 11.8 & 121 & 57.4 & 0.12 & 0.19 & 1.07 & 0.08 & 2.37 & N \\ 
 344 & 5 35 29.6 & 5 36 20 & 77.5 & 4331 & 1.9 & 27.5 & 16.4 & 163 & 74.3 & 0.15 & 0.23 & 1.27 & 0.12 & 1.30 & N \\ 
 345 & 5 35 29.8 & 6 19 48 & 46.0 & 5738 & 3.4 & 31.0 & 14.1 & 175 & 85.5 & 0.17 & 0.29 & 2.20 & 0.13 & 1.47 & N \\ 
 346 & 5 35 29.9 & 6 27 27 & 65.5 & 5681 & 6.1 & 26.8 & 22.9 & 65 & 85.1 & 0.17 & 0.26 & 4.50 & 0.05 & 3.05 & Y \\ 
 347 & 5 35 30.1 & 5 3 6 & 84.1 & 1406 & 5.0 & 17.3 & 5.1 & 135 & 42.3 & 0.08 & 0.28 & 0.94 & 0.13 & 5.17 & N \\ 
 348 & 5 35 30.1 & 5 14 60 & 80.4 & 4556 & 1.7 & 34.1 & 14.5 & 116 & 76.2 & 0.15 & 0.23 & 0.88 & 0.17 & 0.83 & N \\ 
 349 & 5 35 30.2 & 6 12 42 & 59.7 & 3150 & 1.8 & 29.2 & 14.0 & 101 & 63.3 & 0.13 & 0.18 & 0.61 & 0.13 & 1.00 & N \\ 
 350 & 5 35 30.7 & 6 25 6 & 37.7 & 7369 & 2.8 & 25.9 & 16.6 & -170 & 96.9 & 0.19 & 0.34 & 2.82 & 0.15 & 1.30 & N \\ 
 351 & 5 35 30.8 & 5 20 43 & 49.4 & 6806 & 1.8 & 34.7 & 15.0 & -157 & 93.1 & 0.19 & 0.79 & 2.72 & 0.82 & 1.41 & N \\ 
 352 & 5 35 31.0 & 6 1 43 & 55.3 & 9000 & 3.0 & 24.5 & 23.7 & -137 & 107.0 & 0.21 & 0.37 & 2.92 & 0.20 & 0.99 & N \\ 
 353 & 5 35 31.1 & 6 10 26 & 67.9 & 2250 & 2.7 & 20.8 & 7.7 & 134 & 53.5 & 0.11 & 0.33 & 0.46 & 0.49 & 1.24 & N \\ 
 354 & 5 35 31.1 & 6 42 40 & 63.3 & 3375 & 1.5 & 22.3 & 14.0 & 109 & 65.6 & 0.13 & 0.30 & 1.02 & 0.22 & 1.51 & N \\ 
 355 & 5 35 31.2 & 5 57 52 & 57.9 & 7819 & 3.4 & 25.7 & 18.3 & 145 & 99.8 & 0.20 & 0.40 & 2.47 & 0.25 & 1.04 & N \\ 
 356 & 5 35 31.7 & 5 9 48 & 90.5 & 5063 & 4.2 & 28.0 & 14.6 & 115 & 80.3 & 0.16 & 0.38 & 4.29 & 0.10 & 3.46 & N \\ 
 357 & 5 35 31.8 & 6 35 33 & 56.2 & 4163 & 1.9 & 18.8 & 14.9 & 157 & 72.8 & 0.15 & 0.25 & 0.59 & 0.30 & 0.64 & N \\ 
 358 & 5 35 31.9 & 5 54 26 & 57.1 & 3994 & 4.3 & 27.1 & 10.9 & 90 & 71.3 & 0.14 & 0.17 & 2.17 & 0.03 & 2.50 & N \\ 
 359 & 5 35 32.3 & 5 0 60 & 108.5 & 3994 & 1.7 & 22.4 & 10.7 & 74 & 71.3 & 0.14 & 0.69 & 0.76 & 1.71 & 0.88 & N \\ 
 360 & 5 35 32.3 & 5 5 40 & 98.7 & 2025 & 6.1 & 16.1 & 8.8 & 156 & 50.8 & 0.10 & 0.44 & 2.37 & 0.16 & 7.57 & N \\ 
 361 & 5 35 32.3 & 5 11 2 & 86.1 & 5231 & 3.7 & 34.2 & 12.2 & 144 & 81.6 & 0.16 & 0.28 & 2.81 & 0.09 & 2.16 & N \\ 
 362 & 5 35 32.4 & 5 57 23 & 73.0 & 7875 & 1.9 & 35.5 & 17.2 & 100 & 100.1 & 0.20 & 0.25 & 1.26 & 0.19 & 0.52 & N \\ 
 363 & 5 35 32.4 & 6 4 37 & 51.4 & 2925 & 3.5 & 17.6 & 13.5 & -170 & 61.0 & 0.12 & 0.26 & 0.58 & 0.26 & 1.07 & N \\ 
 364 & 5 35 32.5 & 5 25 58 & 95.3 & 2700 & 1.3 & 19.7 & 11.2 & 56 & 58.6 & 0.12 & 0.21 & 0.38 & 0.27 & 0.79 & N \\ 
 365 & 5 35 32.9 & 6 10 0 & 43.1 & 2756 & 1.4 & 20.2 & 11.9 & 102 & 59.2 & 0.12 & 0.20 & 0.18 & 0.53 & 0.36 & N \\ 
 366 & 5 35 33.0 & 5 20 47 & 57.2 & 6581 & 1.9 & 30.6 & 13.3 & 56 & 91.5 & 0.18 & 0.69 & 2.66 & 0.62 & 1.45 & N \\ 
 367 & 5 35 33.1 & 5 20 29 & 69.2 & 5681 & 1.4 & 46.8 & 12.8 & 109 & 85.1 & 0.17 & 0.33 & 1.01 & 0.35 & 0.69 & N \\ 
 368 & 5 35 33.2 & 4 59 37 & 96.3 & 2250 & 5.1 & 21.5 & 7.5 & 176 & 53.5 & 0.11 & 0.23 & 1.59 & 0.07 & 4.34 & N \\ 
 369 & 5 35 33.4 & 5 37 30 & 79.7 & 5513 & 1.7 & 22.3 & 18.0 & 141 & 83.8 & 0.17 & 0.43 & 1.72 & 0.35 & 1.22 & N \\ 
 370 & 5 35 33.4 & 6 2 50 & 58.0 & 3544 & 2.4 & 23.9 & 11.4 & 129 & 67.2 & 0.13 & 0.16 & 0.51 & 0.13 & 0.70 & N \\ 
 371 & 5 35 33.4 & 6 5 20 & 105.8 & 1238 & 1.5 & 11.4 & 6.5 & -173 & 39.7 & 0.08 & 0.20 & 0.12 & 0.48 & 0.83 & N \\ 
 372 & 5 35 33.6 & 6 12 49 & 37.5 & 4275 & 1.8 & 24.1 & 10.9 & 92 & 73.8 & 0.15 & 0.18 & 0.74 & 0.13 & 0.77 & N \\ 
 373 & 5 35 34.0 & 5 56 43 & 51.4 & 2419 & 1.5 & 16.0 & 12.3 & 55 & 55.5 & 0.11 & 0.25 & 0.26 & 0.50 & 0.63 & N \\ 
 374 & 5 35 34.1 & 5 19 39 & 47.4 & 3600 & 1.6 & 20.1 & 12.6 & 165 & 67.7 & 0.14 & 0.23 & 1.09 & 0.12 & 1.47 & N \\ 
 375 & 5 35 34.2 & 6 16 46 & 63.8 & 4669 & 1.9 & 30.4 & 13.2 & 65 & 77.1 & 0.15 & 0.16 & 1.31 & 0.06 & 1.19 & N \\ 
 376 & 5 35 34.3 & 6 2 29 & 68.3 & 2025 & 1.6 & 14.7 & 10.0 & 153 & 50.8 & 0.10 & 0.17 & 0.18 & 0.31 & 0.58 & N \\ 
 377 & 5 35 34.8 & 5 20 55 & 36.1 & 4838 & 1.5 & 34.4 & 16.1 & 65 & 78.5 & 0.16 & 0.24 & 1.08 & 0.17 & 0.93 & N \\ 
 378 & 5 35 35.0 & 5 29 7 & 48.2 & 3994 & 1.4 & 30.4 & 17.6 & 136 & 71.3 & 0.14 & 0.20 & 0.64 & 0.17 & 0.73 & N \\ 
 379 & 5 35 35.0 & 6 5 13 & 47.5 & 2475 & 3.5 & 19.2 & 8.9 & -179 & 56.1 & 0.11 & 0.24 & 0.80 & 0.15 & 1.88 & N \\ 
 380 & 5 35 35.3 & 5 6 57 & 103.9 & 3488 & 3.2 & 20.0 & 12.3 & -170 & 66.6 & 0.13 & 0.32 & 1.57 & 0.17 & 2.21 & N \\ 
 381 & 5 35 35.3 & 5 38 17 & 81.9 & 4388 & 1.7 & 25.0 & 16.0 & 144 & 74.7 & 0.15 & 0.25 & 0.73 & 0.25 & 0.73 & N \\ 
 382 & 5 35 35.3 & 6 11 38 & 64.7 & 4725 & 2.7 & 19.2 & 18.3 & 91 & 77.6 & 0.16 & 0.16 & 1.26 & 0.06 & 1.13 & N \\ 
 383 & 5 35 35.4 & 5 12 30 & 101.5 & 3656 & 1.7 & 23.7 & 12.8 & 88 & 68.2 & 0.14 & 0.24 & 0.60 & 0.26 & 0.79 & N \\ 
 384 & 5 35 35.6 & 5 8 4 & 92.2 & 3488 & 3.0 & 16.6 & 13.7 & 136 & 66.6 & 0.13 & 0.59 & 1.23 & 0.72 & 1.74 & N \\ 
 385 & 5 35 35.7 & 5 47 26 & 30.0 & 2250 & 1.5 & 16.8 & 9.1 & 92 & 53.5 & 0.11 & 0.21 & 0.43 & 0.20 & 1.16 & N \\ 
 386 & 5 35 35.8 & 5 22 20 & 37.5 & 3206 & 1.5 & 22.5 & 12.9 & -178 & 63.9 & 0.13 & 0.32 & 1.46 & 0.16 & 2.34 & N \\ 
 387 & 5 35 35.8 & 5 24 1 & 91.3 & 2756 & 2.4 & 17.6 & 10.1 & 152 & 59.2 & 0.12 & 0.44 & 0.49 & 0.87 & 0.99 & N \\ 
 388 & 5 35 35.8 & 6 20 33 & 69.4 & 2813 & 1.7 & 16.2 & 14.9 & 57 & 59.8 & 0.12 & 0.20 & 0.52 & 0.17 & 1.02 & N \\ 
 389 & 5 35 35.9 & 6 18 11 & 44.8 & 4781 & 3.1 & 20.1 & 13.7 & 77 & 78.0 & 0.16 & 0.25 & 2.00 & 0.09 & 1.76 & N \\ 
 390 & 5 35 35.9 & 6 18 28 & 65.6 & 4500 & 1.5 & 29.9 & 18.5 & 95 & 75.7 & 0.15 & 0.20 & 0.50 & 0.22 & 0.48 & N \\ 
 391 & 5 35 36.1 & 6 4 36 & 59.6 & 5681 & 2.7 & 22.8 & 18.6 & 121 & 85.1 & 0.17 & 0.33 & 1.32 & 0.26 & 0.90 & N \\ 
 392 & 5 35 36.2 & 6 1 40 & 47.5 & 11194 & 2.4 & 30.4 & 27.8 & 69 & 119.4 & 0.24 & 0.30 & 3.09 & 0.13 & 0.76 & N \\ 
 393 & 5 35 36.6 & 5 46 52 & 62.0 & 2138 & 1.3 & 15.8 & 11.5 & 142 & 52.2 & 0.10 & 0.17 & 0.37 & 0.16 & 1.09 & N \\ 
 394 & 5 35 36.7 & 5 18 3 & 64.3 & 3150 & 1.6 & 19.6 & 13.8 & 150 & 63.3 & 0.13 & 0.21 & 0.56 & 0.19 & 0.92 & N \\ 
 395 & 5 35 36.8 & 5 15 50 & 75.8 & 2025 & 1.7 & 13.7 & 8.4 & -174 & 50.8 & 0.10 & 0.49 & 0.65 & 0.70 & 2.08 & N \\ 
 396 & 5 35 36.8 & 6 33 43 & 56.1 & 4950 & 1.7 & 32.6 & 18.1 & 59 & 79.4 & 0.16 & 0.26 & 0.53 & 0.39 & 0.44 & N \\ 
 397 & 5 35 37.2 & 5 23 26 & 99.3 & 2756 & 1.6 & 31.3 & 12.3 & -176 & 59.2 & 0.12 & 0.21 & 0.66 & 0.16 & 1.33 & N \\ 
 398 & 5 35 37.2 & 5 57 33 & 58.7 & 2700 & 2.6 & 18.8 & 9.2 & 149 & 58.6 & 0.12 & 0.30 & 0.70 & 0.28 & 1.46 & N \\ 
 399 & 5 35 37.4 & 6 9 5 & 73.5 & 5344 & 2.8 & 32.2 & 14.4 & 54 & 82.5 & 0.17 & 0.25 & 0.94 & 0.20 & 0.70 & N \\ 
 400 & 5 35 37.5 & 6 31 15 & 57.3 & 1688 & 2.2 & 12.4 & 10.7 & 94 & 46.4 & 0.09 & 0.23 & 0.16 & 0.58 & 0.67 & N \\ 
 401 & 5 35 37.8 & 6 7 18 & 59.0 & 4500 & 3.4 & 23.5 & 17.2 & 141 & 75.7 & 0.15 & 0.30 & 1.15 & 0.23 & 1.10 & N \\ 
 402 & 5 35 37.9 & 5 6 19 & 96.6 & 2475 & 4.8 & 17.6 & 9.0 & -175 & 56.1 & 0.11 & 0.39 & 1.97 & 0.17 & 4.66 & N \\ 
 403 & 5 35 38.3 & 5 15 31 & 88.1 & 4894 & 1.9 & 28.2 & 12.5 & 99 & 78.9 & 0.16 & 0.28 & 1.06 & 0.22 & 0.90 & N \\ 
 404 & 5 35 38.3 & 5 57 49 & 73.0 & 7369 & 1.8 & 33.3 & 16.2 & 50 & 96.9 & 0.19 & 0.33 & 1.37 & 0.29 & 0.63 & N \\ 
 405 & 5 35 38.4 & 6 28 27 & 67.5 & 5794 & 4.7 & 31.3 & 19.7 & 137 & 85.9 & 0.17 & 0.28 & 1.67 & 0.15 & 1.10 & N \\ 
 406 & 5 35 38.6 & 6 38 19 & 65.1 & 8100 & 1.5 & 46.9 & 24.6 & 91 & 101.6 & 0.20 & 0.20 & 2.02 & 0.08 & 0.80 & N \\ 
 407 & 5 35 38.7 & 6 8 6 & 63.5 & 5400 & 3.4 & 26.4 & 16.7 & 75 & 82.9 & 0.17 & 0.26 & 1.36 & 0.16 & 1.00 & N \\ 
 408 & 5 35 38.8 & 5 56 45 & 61.9 & 1913 & 2.8 & 12.1 & 11.3 & 59 & 49.3 & 0.10 & 0.18 & 0.63 & 0.09 & 2.18 & N \\ 
 409 & 5 35 38.8 & 6 47 3 & 48.6 & 6975 & 1.5 & 34.4 & 17.5 & 114 & 94.2 & 0.19 & 0.35 & 1.37 & 0.32 & 0.68 & N \\ 
 410 & 5 35 39.1 & 5 8 27 & 88.4 & 2138 & 2.9 & 15.0 & 8.7 & 137 & 52.2 & 0.10 & 0.37 & 0.62 & 0.45 & 1.81 & N \\ 
 411 & 5 35 39.3 & 5 1 36 & 95.5 & 5288 & 3.7 & 32.9 & 12.4 & -137 & 82.1 & 0.16 & 0.29 & 2.08 & 0.12 & 1.57 & N \\ 
 412 & 5 35 39.6 & 5 17 34 & 71.1 & 3994 & 2.1 & 33.0 & 13.5 & -174 & 71.3 & 0.14 & 0.24 & 1.04 & 0.16 & 1.20 & N \\ 
 413 & 5 35 39.8 & 6 14 17 & 68.3 & 2531 & 3.8 & 13.6 & 11.8 & -160 & 56.8 & 0.11 & 0.24 & 0.88 & 0.14 & 2.00 & N \\ 
 414 & 5 35 40.0 & 5 26 26 & 59.7 & 4500 & 1.8 & 27.0 & 19.0 & 76 & 75.7 & 0.15 & 0.34 & 0.33 & 1.03 & 0.32 & N \\ 
 415 & 5 35 40.0 & 5 54 28 & 61.5 & 5063 & 1.7 & 31.4 & 12.4 & 66 & 80.3 & 0.16 & 0.31 & 1.15 & 0.26 & 0.93 & N \\ 
 416 & 5 35 40.3 & 6 10 47 & 48.0 & 5119 & 2.2 & 28.8 & 12.6 & -155 & 80.7 & 0.16 & 0.32 & 0.79 & 0.41 & 0.63 & N \\ 
 417 & 5 35 40.5 & 5 19 35 & 68.7 & 1913 & 2.1 & 15.1 & 9.2 & -141 & 49.3 & 0.10 & 0.46 & 0.75 & 0.52 & 2.60 & N \\ 
 418 & 5 35 40.6 & 6 5 13 & 71.4 & 11081 & 2.4 & 38.8 & 20.2 & 94 & 118.8 & 0.24 & 0.42 & 3.74 & 0.22 & 0.93 & N \\ 
 419 & 5 35 40.7 & 5 6 52 & 103.4 & 1688 & 3.1 & 13.4 & 8.2 & -167 & 46.4 & 0.09 & 0.21 & 0.69 & 0.11 & 2.89 & N \\ 
 420 & 5 35 40.7 & 6 40 5 & 55.5 & 3150 & 1.9 & 19.1 & 10.9 & 166 & 63.3 & 0.13 & 0.20 & 0.56 & 0.17 & 0.93 & N \\ 
 421 & 5 35 41.0 & 5 59 32 & 75.1 & 2419 & 1.6 & 16.0 & 10.9 & 45 & 55.5 & 0.11 & 0.18 & 0.41 & 0.16 & 1.00 & N \\ 
 422 & 5 35 41.0 & 6 6 57 & 69.1 & 5681 & 2.6 & 27.6 & 15.7 & 132 & 85.1 & 0.17 & 0.29 & 1.15 & 0.24 & 0.78 & N \\ 
 423 & 5 35 41.1 & 5 22 51 & 36.9 & 3994 & 1.7 & 21.1 & 11.3 & 67 & 71.3 & 0.14 & 0.50 & 0.83 & 0.82 & 0.96 & N \\ 
 424 & 5 35 41.3 & 6 10 55 & 67.3 & 4781 & 3.0 & 19.0 & 16.4 & 56 & 78.0 & 0.16 & 0.30 & 1.18 & 0.22 & 1.04 & N \\ 
 425 & 5 35 41.4 & 5 26 53 & 71.0 & 7031 & 1.9 & 41.2 & 15.0 & 121 & 94.6 & 0.19 & 0.31 & 0.76 & 0.45 & 0.38 & N \\ 
 426 & 5 35 41.6 & 6 0 8 & 63.4 & 4725 & 2.5 & 24.1 & 11.6 & -142 & 77.6 & 0.16 & 0.21 & 1.52 & 0.08 & 1.36 & N \\ 
 427 & 5 35 41.7 & 5 20 25 & 49.9 & 2419 & 1.9 & 16.5 & 11.4 & 50 & 55.5 & 0.11 & 0.21 & 0.34 & 0.27 & 0.84 & N \\ 
 428 & 5 35 41.9 & 6 1 34 & 72.4 & 3769 & 1.9 & 27.0 & 12.6 & 54 & 69.3 & 0.14 & 0.26 & 0.95 & 0.19 & 1.19 & N \\ 
 429 & 5 35 42.2 & 6 5 26 & 46.8 & 6244 & 3.1 & 26.1 & 20.3 & 46 & 89.2 & 0.18 & 0.27 & 2.44 & 0.10 & 1.44 & N \\ 
 430 & 5 35 42.3 & 5 20 38 & 61.8 & 5681 & 2.9 & 23.8 & 13.2 & -137 & 85.1 & 0.17 & 0.63 & 3.17 & 0.41 & 2.15 & N \\ 
 431 & 5 35 42.5 & 6 22 55 & 62.1 & 9113 & 3.1 & 44.0 & 20.5 & 74 & 107.7 & 0.22 & 0.26 & 1.29 & 0.21 & 0.43 & N \\ 
 432 & 5 35 43.2 & 5 21 13 & 112.9 & 3150 & 1.9 & 30.2 & 9.0 & 96 & 63.3 & 0.13 & 0.17 & 0.62 & 0.11 & 1.02 & N \\ 
 433 & 5 35 43.5 & 6 32 6 & 54.9 & 4500 & 1.7 & 22.2 & 17.1 & 133 & 75.7 & 0.15 & 0.36 & 0.40 & 0.92 & 0.39 & N \\ 
 434 & 5 35 44.1 & 5 10 39 & 83.9 & 2869 & 2.4 & 24.8 & 9.8 & -148 & 60.4 & 0.12 & 0.23 & 0.53 & 0.23 & 1.00 & N \\ 
 435 & 5 35 44.1 & 6 37 50 & 53.5 & 2138 & 1.9 & 15.6 & 7.8 & 168 & 52.2 & 0.10 & 0.22 & 0.26 & 0.37 & 0.76 & N \\ 
 436 & 5 35 44.3 & 6 8 5 & 58.3 & 6975 & 4.6 & 26.7 & 14.8 & 86 & 94.2 & 0.19 & 0.45 & 4.77 & 0.15 & 2.38 & N \\ 
 437 & 5 35 44.6 & 5 23 42 & 91.0 & 4444 & 1.7 & 27.0 & 18.9 & -175 & 75.2 & 0.15 & 0.15 & 1.15 & 0.06 & 1.13 & N \\ 
 438 & 5 35 44.7 & 6 41 32 & 58.5 & 4613 & 2.5 & 18.1 & 14.9 & 150 & 76.6 & 0.15 & 0.51 & 0.69 & 1.08 & 0.64 & N \\ 
 439 & 5 35 45.2 & 5 28 27 & 71.8 & 3544 & 1.5 & 25.2 & 11.2 & 156 & 67.2 & 0.13 & 0.19 & 0.53 & 0.17 & 0.73 & N \\ 
 440 & 5 35 45.3 & 5 54 42 & 61.6 & 7594 & 1.6 & 46.8 & 17.4 & 112 & 98.3 & 0.20 & 0.24 & 1.26 & 0.17 & 0.55 & N \\ 
 441 & 5 35 45.7 & 6 11 40 & 49.9 & 2700 & 2.0 & 13.9 & 12.1 & -149 & 58.6 & 0.12 & 0.31 & 0.72 & 0.29 & 1.50 & N \\ 
 442 & 5 35 45.9 & 6 18 25 & 65.0 & 3375 & 2.2 & 18.6 & 12.5 & 88 & 65.6 & 0.13 & 0.39 & 0.87 & 0.44 & 1.29 & N \\ 
 443 & 5 35 46.0 & 5 19 39 & 74.8 & 6300 & 2.2 & 20.1 & 17.5 & 65 & 89.6 & 0.18 & 0.54 & 2.59 & 0.39 & 1.50 & N \\ 
 444 & 5 35 46.5 & 6 2 23 & 64.8 & 5794 & 2.5 & 24.2 & 16.7 & 92 & 85.9 & 0.17 & 0.24 & 1.75 & 0.10 & 1.15 & N \\ 
 445 & 5 35 47.7 & 5 21 21 & 65.4 & 2138 & 2.2 & 15.8 & 8.5 & 161 & 52.2 & 0.10 & 0.32 & 1.07 & 0.19 & 3.14 & N \\ 
 446 & 5 35 47.7 & 6 30 10 & 63.3 & 23681 & 5.5 & 49.6 & 28.0 & 64 & 173.6 & 0.35 & 0.45 & 10.24 & 0.13 & 0.82 & N \\ 
 447 & 5 35 47.9 & 6 16 17 & 64.8 & 8719 & 2.2 & 39.5 & 18.6 & 117 & 105.4 & 0.21 & 0.26 & 1.53 & 0.18 & 0.55 & N \\ 
 448 & 5 35 48.1 & 6 25 43 & 39.3 & 19575 & 2.6 & 38.3 & 27.1 & -146 & 157.9 & 0.32 & 0.38 & 3.30 & 0.26 & 0.35 & Y \\ 
 449 & 5 35 48.2 & 6 47 8 & 67.0 & 3150 & 1.6 & 36.3 & 8.7 & 83 & 63.3 & 0.13 & 0.14 & 0.28 & 0.17 & 0.46 & N \\ 
 450 & 5 35 48.7 & 6 27 22 & 66.4 & 3150 & 4.2 & 16.3 & 13.6 & 140 & 63.3 & 0.13 & 0.23 & 1.03 & 0.12 & 1.69 & N \\ 
 451 & 5 35 48.7 & 6 33 5 & 62.0 & 2531 & 2.6 & 20.2 & 11.8 & 52 & 56.8 & 0.11 & 0.21 & 0.26 & 0.36 & 0.59 & N \\ 
 452 & 5 35 48.8 & 5 23 40 & 94.2 & 2756 & 1.6 & 18.3 & 13.9 & -164 & 59.2 & 0.12 & 0.23 & 1.11 & 0.10 & 2.24 & N \\ 
 453 & 5 35 48.9 & 5 51 8 & 74.9 & 3263 & 1.7 & 17.0 & 15.7 & 119 & 64.5 & 0.13 & 0.22 & 0.71 & 0.17 & 1.11 & N \\ 
 454 & 5 35 49.1 & 6 10 11 & 63.6 & 6188 & 4.0 & 21.4 & 17.9 & 108 & 88.8 & 0.18 & 0.41 & 3.42 & 0.16 & 2.04 & N \\ 
 455 & 5 35 49.4 & 6 48 32 & 58.9 & 4613 & 1.5 & 24.2 & 14.9 & 87 & 76.6 & 0.15 & 0.26 & 0.47 & 0.41 & 0.44 & N \\ 
 456 & 5 35 49.5 & 5 24 48 & 31.4 & 2925 & 1.4 & 29.4 & 10.6 & 96 & 61.0 & 0.12 & 0.19 & 1.08 & 0.07 & 1.99 & N \\ 
 457 & 5 35 50.4 & 5 53 3 & 63.8 & 3094 & 1.4 & 26.4 & 10.9 & 164 & 62.8 & 0.13 & 0.25 & 0.80 & 0.18 & 1.34 & N \\ 
 458 & 5 35 50.5 & 5 24 1 & 98.4 & 3769 & 1.6 & 26.0 & 11.6 & 81 & 69.3 & 0.14 & 0.25 & 1.75 & 0.09 & 2.20 & N \\ 
 459 & 5 35 51.4 & 5 20 54 & 73.4 & 5625 & 2.1 & 27.2 & 12.9 & -148 & 84.6 & 0.17 & 0.45 & 1.56 & 0.41 & 1.08 & N \\ 
 460 & 5 35 51.9 & 5 20 51 & 85.8 & 7931 & 1.5 & 29.6 & 18.4 & 87 & 100.5 & 0.20 & 0.55 & 1.55 & 0.74 & 0.64 & N \\ 
 461 & 5 35 51.9 & 6 0 33 & 62.7 & 4613 & 1.9 & 18.1 & 15.9 & 83 & 76.6 & 0.15 & 0.34 & 1.35 & 0.24 & 1.26 & N \\ 
 462 & 5 35 52.1 & 6 46 4 & 44.3 & 4444 & 3.2 & 23.9 & 14.3 & 134 & 75.2 & 0.15 & 0.22 & 0.84 & 0.16 & 0.83 & N \\ 
 463 & 5 35 52.2 & 6 4 43 & 66.0 & 2363 & 2.9 & 27.7 & 7.2 & 89 & 54.8 & 0.11 & 0.15 & 0.66 & 0.07 & 1.66 & N \\ 
 464 & 5 35 52.2 & 6 45 39 & 49.9 & 1913 & 1.8 & 19.7 & 8.3 & 122 & 49.3 & 0.10 & 0.18 & 0.16 & 0.38 & 0.55 & N \\ 
 465 & 5 35 52.3 & 6 34 49 & 68.3 & 19069 & 4.8 & 39.2 & 31.7 & 74 & 155.8 & 0.31 & 0.28 & 8.94 & 0.05 & 0.99 & Y \\ 
 466 & 5 35 52.8 & 5 55 23 & 65.9 & 4275 & 1.9 & 22.7 & 16.1 & 155 & 73.8 & 0.15 & 0.46 & 1.41 & 0.42 & 1.47 & N \\ 
 467 & 5 35 53.4 & 5 42 12 & 59.6 & 19406 & 3.6 & 36.5 & 31.0 & -141 & 157.2 & 0.32 & 0.55 & 13.25 & 0.13 & 1.43 & N \\ 
 468 & 5 35 53.5 & 6 24 29 & 68.8 & 6413 & 5.1 & 24.1 & 16.6 & 180 & 90.4 & 0.18 & 0.32 & 2.50 & 0.14 & 1.42 & N \\ 
 469 & 5 35 53.5 & 6 34 45 & 56.6 & 8156 & 3.1 & 42.4 & 16.2 & 56 & 101.9 & 0.20 & 0.28 & 1.18 & 0.26 & 0.47 & N \\ 
 470 & 5 35 53.9 & 6 10 27 & 62.4 & 4275 & 3.9 & 27.3 & 12.2 & -135 & 73.8 & 0.15 & 0.39 & 2.10 & 0.21 & 2.18 & N \\ 
 471 & 5 35 54.2 & 5 57 53 & 59.7 & 3713 & 1.5 & 18.9 & 14.3 & 168 & 68.8 & 0.14 & 0.24 & 0.93 & 0.17 & 1.19 & N \\ 
 472 & 5 35 54.4 & 6 4 32 & 84.8 & 4275 & 1.6 & 23.8 & 20.2 & -166 & 73.8 & 0.15 & 0.28 & 0.67 & 0.34 & 0.70 & N \\ 
 473 & 5 35 54.7 & 6 15 54 & 66.4 & 3938 & 2.4 & 20.2 & 15.2 & 62 & 70.8 & 0.14 & 0.33 & 0.71 & 0.41 & 0.84 & N \\ 
 474 & 5 35 54.7 & 6 32 22 & 42.2 & 2700 & 1.5 & 18.9 & 13.5 & 86 & 58.6 & 0.12 & 0.33 & 0.13 & 1.87 & 0.26 & N \\ 
 475 & 5 35 54.7 & 6 44 27 & 64.5 & 13163 & 1.5 & 50.5 & 21.6 & 80 & 129.5 & 0.26 & 0.31 & 1.34 & 0.34 & 0.26 & N \\ 
 476 & 5 35 55.1 & 6 26 12 & 67.8 & 5288 & 3.5 & 31.6 & 14.8 & -179 & 82.1 & 0.16 & 0.41 & 1.50 & 0.35 & 1.14 & N \\ 
 477 & 5 35 55.1 & 6 42 49 & 113.2 & 2700 & 1.6 & 20.6 & 9.9 & -138 & 58.6 & 0.12 & 0.25 & 0.13 & 1.09 & 0.27 & N \\ 
 478 & 5 35 55.2 & 6 7 12 & 60.4 & 4331 & 1.7 & 25.2 & 15.0 & 88 & 74.3 & 0.15 & 0.48 & 0.82 & 0.79 & 0.84 & N \\ 
 479 & 5 35 55.4 & 5 32 22 & 53.1 & 74475 & 2.9 & 99.1 & 43.2 & 65 & 307.9 & 0.62 & 0.49 & 45.95 & 0.06 & 0.66 & N \\ 
 480 & 5 35 55.6 & 6 15 51 & 53.5 & 2306 & 1.4 & 18.7 & 9.7 & 60 & 54.2 & 0.11 & 0.19 & 0.16 & 0.46 & 0.42 & N \\ 
 481 & 5 35 55.8 & 5 44 55 & 57.5 & 4106 & 1.5 & 40.2 & 14.9 & 176 & 72.3 & 0.15 & 0.17 & 2.12 & 0.04 & 2.34 & N \\ 
 482 & 5 35 55.8 & 6 48 27 & 66.4 & 5006 & 1.6 & 44.6 & 10.0 & 50 & 79.8 & 0.16 & 0.40 & 0.31 & 1.59 & 0.26 & N \\ 
 483 & 5 35 56.0 & 6 40 8 & 52.2 & 5119 & 1.7 & 33.0 & 19.2 & 136 & 80.7 & 0.16 & 0.18 & 0.59 & 0.17 & 0.47 & N \\ 
 484 & 5 35 57.0 & 5 47 16 & 59.7 & 4725 & 1.6 & 29.2 & 18.0 & -152 & 77.6 & 0.16 & 0.38 & 2.10 & 0.21 & 1.88 & N \\ 
 485 & 5 35 57.5 & 6 6 39 & 69.0 & 8213 & 1.8 & 37.6 & 23.2 & 56 & 102.3 & 0.21 & 0.40 & 1.84 & 0.34 & 0.72 & N \\ 
 486 & 5 35 57.5 & 6 32 28 & 62.7 & 11475 & 4.6 & 36.9 & 18.7 & 87 & 120.9 & 0.24 & 0.40 & 3.35 & 0.22 & 0.79 & N \\ 
 487 & 5 35 58.6 & 6 32 4 & 70.8 & 4500 & 4.1 & 18.9 & 14.7 & 126 & 75.7 & 0.15 & 0.23 & 1.29 & 0.12 & 1.24 & N \\ 
 488 & 5 35 58.8 & 6 21 55 & 54.2 & 10238 & 1.9 & 44.1 & 19.1 & 117 & 114.2 & 0.23 & 0.33 & 1.28 & 0.36 & 0.36 & N \\ 
 489 & 5 35 59.3 & 5 20 27 & 90.0 & 1519 & 1.5 & 14.1 & 9.2 & 175 & 44.0 & 0.09 & 0.21 & 0.30 & 0.24 & 1.45 & N \\ 
 490 & 5 35 59.3 & 6 23 50 & 65.7 & 2250 & 4.0 & 13.8 & 11.2 & -164 & 53.5 & 0.11 & 0.21 & 0.46 & 0.19 & 1.25 & N \\ 
 491 & 5 35 59.8 & 6 40 24 & 42.9 & 3600 & 1.5 & 24.2 & 12.1 & -164 & 67.7 & 0.14 & 0.38 & 0.37 & 1.00 & 0.50 & N \\ 
 492 & 5 35 59.9 & 6 38 42 & 65.3 & 7763 & 2.8 & 34.9 & 14.9 & -143 & 99.4 & 0.20 & 0.23 & 1.09 & 0.18 & 0.46 & N \\ 
 493 & 5 35 60.0 & 6 39 24 & 56.7 & 4163 & 1.7 & 30.9 & 11.1 & 87 & 72.8 & 0.15 & 0.17 & 0.33 & 0.25 & 0.35 & N \\ 
 494 & 5 36 0.1 & 5 20 16 & 86.4 & 6356 & 1.5 & 34.3 & 19.5 & 61 & 90.0 & 0.18 & 0.30 & 1.26 & 0.24 & 0.73 & N \\ 
 495 & 5 36 0.1 & 6 37 53 & 48.5 & 3938 & 2.5 & 29.7 & 10.2 & -172 & 70.8 & 0.14 & 0.26 & 0.42 & 0.43 & 0.49 & N \\ 
 496 & 5 36 0.4 & 6 1 44 & 67.1 & 2869 & 1.8 & 21.3 & 14.0 & 135 & 60.4 & 0.12 & 0.20 & 0.76 & 0.12 & 1.44 & N \\ 
 497 & 5 36 0.9 & 5 21 54 & 101.5 & 6356 & 1.5 & 27.7 & 16.7 & 78 & 90.0 & 0.18 & 0.37 & 2.35 & 0.20 & 1.35 & N \\ 
 498 & 5 36 0.9 & 6 3 58 & 42.0 & 2363 & 1.6 & 16.4 & 9.8 & -166 & 54.8 & 0.11 & 0.19 & 0.45 & 0.16 & 1.15 & N \\ 
 499 & 5 36 1.1 & 6 36 34 & 65.9 & 2306 & 1.8 & 19.2 & 9.9 & 139 & 54.2 & 0.11 & 0.21 & 0.20 & 0.48 & 0.51 & N \\ 
 500 & 5 36 1.7 & 6 35 25 & 54.1 & 8381 & 2.7 & 28.3 & 23.2 & 108 & 103.3 & 0.21 & 0.34 & 1.24 & 0.36 & 0.47 & N \\ 
 501 & 5 36 1.9 & 6 13 59 & 66.2 & 6356 & 3.4 & 25.0 & 14.7 & 45 & 90.0 & 0.18 & 0.46 & 2.08 & 0.35 & 1.19 & N \\ 
 502 & 5 36 1.9 & 6 44 23 & 49.4 & 4613 & 4.6 & 24.9 & 14.8 & 74 & 76.6 & 0.15 & 0.24 & 1.05 & 0.15 & 0.97 & N \\ 
 503 & 5 36 2.0 & 6 4 28 & 93.1 & 4613 & 1.4 & 31.7 & 17.4 & 173 & 76.6 & 0.15 & 0.23 & 1.34 & 0.11 & 1.24 & N \\ 
 504 & 5 36 2.0 & 6 38 7 & 56.3 & 2813 & 1.8 & 20.9 & 10.1 & -164 & 59.8 & 0.12 & 0.37 & 0.24 & 1.25 & 0.47 & N \\ 
 505 & 5 36 2.2 & 5 55 37 & 57.9 & 3994 & 1.5 & 29.2 & 12.5 & 96 & 71.3 & 0.14 & 0.37 & 1.38 & 0.27 & 1.59 & N \\ 
 506 & 5 36 2.3 & 6 12 41 & 69.3 & 1969 & 4.0 & 15.1 & 8.5 & 97 & 50.1 & 0.10 & 0.31 & 0.67 & 0.27 & 2.23 & N \\ 
 507 & 5 36 3.1 & 6 44 38 & 64.3 & 2025 & 2.1 & 20.5 & 8.7 & 149 & 50.8 & 0.10 & 0.20 & 0.13 & 0.56 & 0.43 & N \\ 
 508 & 5 36 3.2 & 6 24 43 & 52.0 & 3544 & 2.2 & 18.8 & 11.7 & -175 & 67.2 & 0.13 & 0.38 & 0.33 & 1.11 & 0.46 & N \\ 
 509 & 5 36 3.6 & 5 37 51 & 54.3 & 13331 & 1.6 & 46.2 & 23.8 & 173 & 130.3 & 0.26 & 0.96 & 5.53 & 0.82 & 1.04 & N \\ 
 510 & 5 36 3.9 & 6 31 19 & 55.1 & 5906 & 1.6 & 45.3 & 16.1 & 148 & 86.7 & 0.17 & 0.17 & 0.33 & 0.27 & 0.21 & N \\ 
 511 & 5 36 4.2 & 5 56 25 & 54.1 & 11869 & 1.6 & 39.0 & 26.0 & 127 & 122.9 & 0.25 & 0.54 & 4.43 & 0.31 & 1.00 & N \\ 
 512 & 5 36 4.2 & 6 19 23 & 74.6 & 3544 & 1.7 & 20.4 & 12.3 & 86 & 67.2 & 0.13 & 0.21 & 0.41 & 0.27 & 0.57 & N \\ 
 513 & 5 36 4.6 & 6 47 15 & 75.9 & 2475 & 1.4 & 27.2 & 10.0 & 77 & 56.1 & 0.11 & 0.18 & 0.13 & 0.51 & 0.30 & N \\ 
 514 & 5 36 4.7 & 6 29 16 & 63.0 & 6019 & 2.7 & 44.3 & 12.2 & 50 & 87.5 & 0.18 & 0.26 & 0.71 & 0.33 & 0.44 & N \\ 
 515 & 5 36 4.8 & 6 46 30 & 47.1 & 12206 & 4.4 & 38.2 & 22.2 & 74 & 124.7 & 0.25 & 0.19 & 3.33 & 0.05 & 0.72 & N \\ 
 516 & 5 36 5.0 & 6 18 2 & 67.9 & 6131 & 1.6 & 33.0 & 19.7 & 67 & 88.4 & 0.18 & 0.38 & 0.61 & 0.79 & 0.37 & N \\ 
 517 & 5 36 5.0 & 6 33 58 & 69.8 & 4444 & 2.2 & 20.7 & 15.5 & 133 & 75.2 & 0.15 & 0.23 & 0.59 & 0.26 & 0.58 & N \\ 
 518 & 5 36 5.0 & 6 39 3 & 54.9 & 2756 & 1.8 & 20.0 & 9.7 & 67 & 59.2 & 0.12 & 0.24 & 0.38 & 0.33 & 0.77 & N \\ 
 519 & 5 36 5.1 & 5 41 58 & 61.9 & 3994 & 1.9 & 20.3 & 12.8 & -160 & 71.3 & 0.14 & 0.24 & 1.37 & 0.11 & 1.58 & N \\ 
 520 & 5 36 5.4 & 6 40 50 & 63.4 & 8550 & 2.7 & 25.5 & 18.4 & 48 & 104.3 & 0.21 & 0.33 & 1.88 & 0.22 & 0.69 & N \\ 
 521 & 5 36 5.7 & 6 37 16 & 48.7 & 3488 & 2.9 & 17.9 & 14.2 & 77 & 66.6 & 0.13 & 0.19 & 0.95 & 0.10 & 1.34 & N \\ 
 522 & 5 36 6.3 & 6 11 27 & 67.2 & 17044 & 4.7 & 40.8 & 30.5 & -147 & 147.3 & 0.30 & 0.53 & 8.24 & 0.19 & 1.08 & N \\ 
 523 & 5 36 6.7 & 6 32 44 & 76.4 & 6525 & 1.9 & 28.3 & 16.9 & 54 & 91.1 & 0.18 & 0.39 & 0.92 & 0.57 & 0.51 & N \\ 
 524 & 5 36 7.1 & 6 42 44 & 47.6 & 2869 & 1.8 & 19.3 & 10.9 & 145 & 60.4 & 0.12 & 0.22 & 0.36 & 0.31 & 0.67 & N \\ 
 525 & 5 36 7.1 & 6 44 59 & 69.2 & 2194 & 3.3 & 14.4 & 10.7 & 97 & 52.9 & 0.11 & 0.18 & 0.35 & 0.19 & 0.99 & N \\ 
 526 & 5 36 7.4 & 6 17 45 & 50.4 & 5231 & 1.7 & 28.5 & 15.4 & 83 & 81.6 & 0.16 & 0.26 & 0.38 & 0.58 & 0.29 & N \\ 
 527 & 5 36 7.5 & 6 41 53 & 51.3 & 3375 & 1.9 & 15.5 & 14.1 & 75 & 65.6 & 0.13 & 0.42 & 0.52 & 0.84 & 0.76 & N \\ 
 528 & 5 36 7.6 & 6 43 24 & 97.9 & 2475 & 1.6 & 26.8 & 9.1 & 68 & 56.1 & 0.11 & 0.16 & 0.18 & 0.32 & 0.43 & N \\ 
 529 & 5 36 7.8 & 6 26 23 & 62.1 & 2588 & 1.6 & 21.5 & 9.1 & 118 & 57.4 & 0.12 & 0.33 & 0.15 & 1.61 & 0.33 & N \\ 
 530 & 5 36 7.8 & 6 46 22 & 65.7 & 3881 & 3.8 & 22.3 & 12.3 & 162 & 70.3 & 0.14 & 0.23 & 1.07 & 0.13 & 1.29 & N \\ 
 531 & 5 36 7.9 & 5 39 24 & 60.3 & 7875 & 1.7 & 41.3 & 16.7 & 45 & 100.1 & 0.20 & 0.41 & 2.89 & 0.22 & 1.20 & N \\ 
 532 & 5 36 8.1 & 6 26 50 & 49.7 & 5119 & 2.2 & 21.9 & 17.8 & 166 & 80.7 & 0.16 & 0.22 & 0.45 & 0.33 & 0.36 & N \\ 
 533 & 5 36 8.6 & 6 37 35 & 60.8 & 2700 & 1.6 & 27.0 & 10.0 & 144 & 58.6 & 0.12 & 0.28 & 0.27 & 0.66 & 0.56 & N \\ 
 534 & 5 36 8.9 & 6 0 0 & 56.8 & 3825 & 1.5 & 20.2 & 14.3 & -165 & 69.8 & 0.14 & 0.38 & 1.55 & 0.25 & 1.91 & N \\ 
 535 & 5 36 9.1 & 5 23 14 & 69.6 & 14400 & 2.0 & 30.7 & 25.6 & 179 & 135.4 & 0.27 & 0.65 & 9.57 & 0.23 & 1.61 & N \\ 
 536 & 5 36 9.1 & 5 36 52 & 55.3 & 2475 & 1.6 & 17.9 & 9.2 & -140 & 56.1 & 0.11 & 0.49 & 0.97 & 0.53 & 2.28 & N \\ 
 537 & 5 36 9.1 & 5 41 17 & 57.0 & 2813 & 2.3 & 20.8 & 7.5 & 99 & 59.8 & 0.12 & 0.46 & 0.75 & 0.64 & 1.47 & N \\ 
 538 & 5 36 9.2 & 6 15 51 & 60.7 & 16706 & 3.7 & 40.6 & 26.6 & 81 & 145.8 & 0.29 & 0.33 & 4.94 & 0.12 & 0.66 & N \\ 
 539 & 5 36 9.6 & 5 21 10 & 82.0 & 5288 & 1.5 & 24.6 & 14.2 & 69 & 82.1 & 0.16 & 0.40 & 1.66 & 0.31 & 1.26 & N \\ 
 540 & 5 36 10.0 & 6 33 57 & 57.2 & 13781 & 3.1 & 45.2 & 21.9 & 71 & 132.5 & 0.27 & 0.61 & 3.80 & 0.49 & 0.68 & N \\ 
 541 & 5 36 10.1 & 6 26 52 & 66.6 & 4613 & 1.6 & 26.4 & 14.5 & 175 & 76.6 & 0.15 & 0.27 & 0.28 & 0.74 & 0.26 & N \\ 
 542 & 5 36 10.4 & 6 19 56 & 70.0 & 3094 & 1.4 & 22.3 & 13.1 & 61 & 62.8 & 0.13 & 0.20 & 0.47 & 0.20 & 0.79 & N \\ 
 543 & 5 36 10.8 & 6 9 26 & 72.5 & 6919 & 1.7 & 33.0 & 17.3 & -162 & 93.9 & 0.19 & 0.27 & 1.20 & 0.21 & 0.60 & N \\ 
 544 & 5 36 11.5 & 6 23 20 & 42.0 & 3206 & 4.1 & 21.1 & 11.3 & 130 & 63.9 & 0.13 & 0.20 & 0.79 & 0.12 & 1.27 & N \\ 
 545 & 5 36 12.3 & 6 28 35 & 69.1 & 2925 & 1.5 & 18.1 & 15.7 & 134 & 61.0 & 0.12 & 0.24 & 0.14 & 0.98 & 0.25 & N \\ 
 546 & 5 36 12.9 & 6 23 15 & 48.1 & 4725 & 4.4 & 20.6 & 16.2 & 78 & 77.6 & 0.16 & 0.24 & 1.49 & 0.11 & 1.33 & N \\ 
 547 & 5 36 12.9 & 6 29 60 & 47.6 & 9394 & 3.2 & 34.7 & 20.7 & 138 & 109.4 & 0.22 & 0.35 & 1.63 & 0.32 & 0.52 & N \\ 
 548 & 5 36 14.2 & 6 46 58 & 59.3 & 14344 & 5.5 & 49.4 & 18.0 & 112 & 135.1 & 0.27 & 0.33 & 8.33 & 0.07 & 1.41 & N \\ 
 549 & 5 36 14.3 & 6 17 22 & 73.5 & 3319 & 1.4 & 20.1 & 16.0 & 61 & 65.0 & 0.13 & 0.19 & 0.25 & 0.37 & 0.38 & N \\ 
 550 & 5 36 14.9 & 5 53 58 & 67.0 & 5963 & 1.7 & 25.9 & 14.8 & 74 & 87.1 & 0.17 & 0.58 & 1.66 & 0.68 & 1.05 & N \\ 
 551 & 5 36 15.2 & 6 35 38 & 67.9 & 3375 & 2.6 & 19.6 & 11.5 & 85 & 65.6 & 0.13 & 0.18 & 0.45 & 0.17 & 0.66 & N \\ 
 552 & 5 36 15.8 & 6 44 34 & 72.7 & 4838 & 4.3 & 19.5 & 17.7 & 168 & 78.5 & 0.16 & 0.36 & 1.75 & 0.22 & 1.52 & N \\ 
 553 & 5 36 15.9 & 6 31 51 & 57.1 & 2250 & 3.4 & 13.9 & 10.2 & 119 & 53.5 & 0.11 & 0.17 & 0.55 & 0.10 & 1.51 & N \\ 
 554 & 5 36 15.9 & 6 37 55 & 65.8 & 12825 & 4.3 & 43.8 & 18.6 & 64 & 127.8 & 0.26 & 0.37 & 4.86 & 0.14 & 0.97 & Y \\ 
 555 & 5 36 16.1 & 6 34 39 & 50.4 & 2869 & 2.4 & 19.7 & 9.7 & 56 & 60.4 & 0.12 & 0.32 & 0.51 & 0.47 & 0.97 & N \\ 
 556 & 5 36 16.3 & 6 36 37 & 46.0 & 1350 & 1.7 & 9.6 & 8.0 & 147 & 41.5 & 0.08 & 0.18 & 0.09 & 0.57 & 0.53 & N \\ 
 557 & 5 36 16.6 & 6 42 54 & 46.0 & 10913 & 1.9 & 42.7 & 20.4 & 173 & 117.9 & 0.24 & 0.46 & 1.36 & 0.68 & 0.35 & N \\ 
 558 & 5 36 17.0 & 6 35 39 & 56.6 & 3263 & 2.3 & 16.9 & 13.4 & -144 & 64.5 & 0.13 & 0.25 & 0.51 & 0.30 & 0.80 & N \\ 
 559 & 5 36 17.3 & 6 48 31 & 44.0 & 9956 & 4.0 & 30.8 & 24.3 & 179 & 112.6 & 0.23 & 0.29 & 4.31 & 0.08 & 1.26 & N \\ 
 560 & 5 36 17.4 & 6 36 47 & 53.5 & 3994 & 2.3 & 18.7 & 14.3 & 67 & 71.3 & 0.14 & 0.41 & 0.69 & 0.66 & 0.80 & N \\ 
 561 & 5 36 18.0 & 6 40 7 & 48.2 & 5175 & 2.8 & 27.0 & 15.4 & 101 & 81.2 & 0.16 & 0.33 & 0.80 & 0.43 & 0.63 & N \\ 
 562 & 5 36 18.5 & 6 5 45 & 63.6 & 2250 & 1.5 & 19.0 & 9.6 & 156 & 53.5 & 0.11 & 0.25 & 0.53 & 0.25 & 1.44 & N \\ 
 563 & 5 36 18.5 & 6 18 18 & 58.3 & 2194 & 1.7 & 20.3 & 9.3 & -154 & 52.9 & 0.11 & 0.22 & 0.29 & 0.35 & 0.81 & N \\ 
 564 & 5 36 18.7 & 6 45 23 & 69.2 & 2588 & 4.4 & 23.1 & 8.5 & 160 & 57.4 & 0.12 & 0.22 & 1.22 & 0.09 & 2.69 & Y \\ 
 565 & 5 36 19.0 & 6 48 8 & 78.4 & 2081 & 2.7 & 17.9 & 10.0 & 143 & 51.5 & 0.10 & 0.30 & 0.53 & 0.32 & 1.63 & N \\ 
 566 & 5 36 19.4 & 6 30 52 & 56.5 & 2756 & 3.1 & 19.2 & 10.0 & 148 & 59.2 & 0.12 & 0.19 & 0.53 & 0.15 & 1.07 & N \\ 
 567 & 5 36 19.8 & 5 52 49 & 48.8 & 3206 & 1.4 & 25.4 & 17.0 & 172 & 63.9 & 0.13 & 0.27 & 0.56 & 0.32 & 0.89 & N \\ 
 568 & 5 36 20.1 & 6 35 25 & 53.9 & 2419 & 2.6 & 16.4 & 12.2 & 55 & 55.5 & 0.11 & 0.19 & 0.45 & 0.17 & 1.09 & N \\ 
 569 & 5 36 20.3 & 6 12 38 & 60.2 & 3881 & 4.7 & 36.9 & 7.4 & 59 & 70.3 & 0.14 & 0.18 & 2.09 & 0.04 & 2.52 & N \\ 
 570 & 5 36 20.3 & 6 30 37 & 47.0 & 11475 & 3.6 & 30.0 & 25.2 & -142 & 120.9 & 0.24 & 0.36 & 3.44 & 0.17 & 0.81 & N \\ 
 571 & 5 36 21.0 & 6 17 48 & 65.7 & 4556 & 2.3 & 31.4 & 10.8 & 97 & 76.2 & 0.15 & 0.29 & 0.78 & 0.31 & 0.74 & N \\ 
 572 & 5 36 21.0 & 6 20 49 & 76.3 & 2475 & 1.5 & 18.8 & 11.0 & 138 & 56.1 & 0.11 & 0.20 & 0.20 & 0.43 & 0.47 & N \\ 
 573 & 5 36 21.1 & 6 33 19 & 47.8 & 5738 & 3.1 & 38.0 & 11.5 & 77 & 85.5 & 0.17 & 0.41 & 1.49 & 0.37 & 1.00 & N \\ 
 574 & 5 36 21.6 & 6 9 24 & 65.1 & 5006 & 2.9 & 26.8 & 15.4 & 179 & 79.8 & 0.16 & 0.24 & 0.74 & 0.23 & 0.61 & N \\ 
 575 & 5 36 22.1 & 6 35 38 & 49.0 & 3488 & 3.1 & 32.4 & 9.5 & 97 & 66.6 & 0.13 & 0.22 & 1.01 & 0.12 & 1.42 & N \\ 
 576 & 5 36 22.6 & 5 55 38 & 59.6 & 6075 & 5.1 & 27.7 & 13.9 & 63 & 87.9 & 0.18 & 0.36 & 6.32 & 0.07 & 3.88 & N \\ 
 577 & 5 36 22.6 & 6 46 24 & 80.9 & 5063 & 5.2 & 21.0 & 12.6 & 120 & 80.3 & 0.16 & 0.46 & 9.31 & 0.07 & 7.52 & Y \\ 
 578 & 5 36 22.9 & 6 19 37 & 40.7 & 11869 & 2.2 & 38.1 & 25.0 & -172 & 122.9 & 0.25 & 0.33 & 2.29 & 0.22 & 0.51 & N \\ 
 579 & 5 36 22.9 & 6 47 22 & 43.7 & 2306 & 2.6 & 18.5 & 8.0 & 100 & 54.2 & 0.11 & 0.27 & 0.88 & 0.17 & 2.30 & N \\ 
 580 & 5 36 23.1 & 6 43 51 & 47.9 & 7481 & 1.7 & 35.5 & 26.9 & 91 & 97.6 & 0.20 & 0.34 & 0.77 & 0.54 & 0.35 & N \\ 
 581 & 5 36 23.5 & 5 59 35 & 61.9 & 3994 & 2.1 & 22.2 & 13.8 & -163 & 71.3 & 0.14 & 0.37 & 0.76 & 0.49 & 0.88 & N \\ 
 582 & 5 36 23.9 & 6 24 6 & 46.4 & 49444 & 6.7 & 63.5 & 51.0 & 164 & 250.9 & 0.50 & 0.78 & 83.99 & 0.07 & 2.22 & Y \\ 
 583 & 5 36 25.2 & 6 14 28 & 62.5 & 4838 & 4.9 & 34.9 & 9.4 & 46 & 78.5 & 0.16 & 0.37 & 5.26 & 0.08 & 4.55 & N \\ 
 584 & 5 36 25.4 & 6 47 19 & 60.4 & 6975 & 2.2 & 37.4 & 14.2 & 74 & 94.2 & 0.19 & 0.61 & 1.81 & 0.73 & 0.90 & Y \\ 
 585 & 5 36 25.7 & 6 44 29 & 66.1 & 9844 & 5.2 & 33.6 & 18.1 & 179 & 112.0 & 0.22 & 0.55 & 8.34 & 0.15 & 2.48 & N \\ 
 586 & 5 36 25.8 & 6 39 42 & 50.0 & 5063 & 2.1 & 20.8 & 15.5 & -180 & 80.3 & 0.16 & 0.30 & 1.24 & 0.22 & 1.00 & N \\ 
 587 & 5 36 26.0 & 6 7 5 & 62.7 & 5231 & 4.5 & 29.3 & 13.1 & 103 & 81.6 & 0.16 & 0.41 & 1.38 & 0.37 & 1.06 & N \\ 
 588 & 5 36 26.1 & 6 42 6 & 67.2 & 5231 & 3.8 & 36.7 & 13.7 & 61 & 81.6 & 0.16 & 0.29 & 1.42 & 0.18 & 1.09 & N \\ 
 589 & 5 36 26.3 & 6 15 22 & 44.2 & 2306 & 1.5 & 13.3 & 11.5 & 66 & 54.2 & 0.11 & 0.18 & 0.17 & 0.40 & 0.45 & N \\ 
 590 & 5 36 26.9 & 6 22 0 & 77.0 & 2756 & 2.0 & 15.4 & 11.6 & 87 & 59.2 & 0.12 & 0.33 & 0.46 & 0.53 & 0.92 & N \\ 
 591 & 5 36 27.0 & 6 20 44 & 61.6 & 6356 & 2.5 & 38.5 & 14.5 & 161 & 90.0 & 0.18 & 0.26 & 1.16 & 0.20 & 0.66 & N \\ 
 592 & 5 36 28.0 & 6 29 19 & 50.9 & 2194 & 2.5 & 14.2 & 11.3 & 169 & 52.9 & 0.11 & 0.19 & 0.25 & 0.28 & 0.71 & N \\ 
 593 & 5 36 28.7 & 6 46 36 & 72.0 & 1575 & 2.0 & 11.3 & 8.9 & 128 & 44.8 & 0.09 & 0.20 & 0.30 & 0.23 & 1.39 & N \\ 
 594 & 5 36 29.5 & 6 48 19 & 42.4 & 1913 & 3.2 & 14.1 & 8.8 & 123 & 49.3 & 0.10 & 0.22 & 0.64 & 0.15 & 2.22 & N \\ 
 595 & 5 36 30.5 & 6 10 7 & 45.9 & 10013 & 2.1 & 47.2 & 21.4 & 94 & 112.9 & 0.23 & 0.45 & 0.77 & 1.15 & 0.22 & N \\ 
 596 & 5 36 30.6 & 6 40 26 & 48.2 & 3713 & 1.8 & 23.7 & 11.9 & -163 & 68.8 & 0.14 & 0.18 & 0.44 & 0.20 & 0.56 & N \\ 
 597 & 5 36 30.7 & 6 21 8 & 77.3 & 2475 & 3.3 & 16.0 & 13.1 & 92 & 56.1 & 0.11 & 0.22 & 0.65 & 0.16 & 1.53 & N \\ 
 598 & 5 36 30.8 & 6 46 40 & 44.8 & 2250 & 3.2 & 19.3 & 9.2 & 85 & 53.5 & 0.11 & 0.21 & 0.44 & 0.21 & 1.20 & N \\ 
 599 & 5 36 31.1 & 6 15 47 & 60.4 & 3094 & 4.9 & 26.8 & 7.7 & -138 & 62.8 & 0.13 & 0.25 & 2.04 & 0.07 & 3.45 & N \\ 
 600 & 5 36 31.5 & 6 41 8 & 71.0 & 2531 & 1.6 & 21.1 & 9.3 & 118 & 56.8 & 0.11 & 0.20 & 0.23 & 0.38 & 0.53 & N \\ 
 601 & 5 36 31.7 & 6 2 2 & 59.8 & 11813 & 7.0 & 35.5 & 28.0 & 72 & 122.6 & 0.25 & 0.28 & 12.73 & 0.03 & 2.88 & Y \\ 
 602 & 5 36 32.1 & 6 33 1 & 52.2 & 3825 & 1.5 & 24.0 & 13.3 & 52 & 69.8 & 0.14 & 0.30 & 0.85 & 0.28 & 1.05 & N \\ 
 603 & 5 36 32.1 & 6 35 45 & 54.4 & 8325 & 1.6 & 55.6 & 17.1 & 99 & 103.0 & 0.21 & 0.16 & 1.09 & 0.10 & 0.42 & N \\ 
 604 & 5 36 32.7 & 6 39 31 & 67.1 & 2925 & 2.4 & 21.3 & 12.6 & 165 & 61.0 & 0.12 & 0.28 & 0.55 & 0.33 & 1.00 & N \\ 
 605 & 5 36 33.1 & 6 26 32 & 51.1 & 3319 & 4.2 & 20.3 & 12.0 & -168 & 65.0 & 0.13 & 0.21 & 1.63 & 0.07 & 2.47 & N \\ 
 606 & 5 36 33.7 & 6 20 45 & 64.3 & 6581 & 2.8 & 27.9 & 16.9 & 81 & 91.5 & 0.18 & 0.48 & 1.31 & 0.61 & 0.71 & N \\ 
 607 & 5 36 33.7 & 6 22 9 & 74.5 & 4556 & 3.6 & 24.5 & 13.5 & 87 & 76.2 & 0.15 & 0.19 & 1.05 & 0.10 & 0.99 & N \\ 
 608 & 5 36 34.0 & 6 23 48 & 73.0 & 1856 & 2.0 & 12.8 & 9.2 & -178 & 48.6 & 0.10 & 0.20 & 0.13 & 0.55 & 0.49 & N \\ 
 609 & 5 36 34.1 & 6 18 47 & 72.0 & 2700 & 1.7 & 19.3 & 11.3 & 131 & 58.6 & 0.12 & 0.19 & 0.28 & 0.29 & 0.59 & N \\ 
 610 & 5 36 35.1 & 6 6 34 & 42.3 & 6525 & 3.2 & 22.7 & 18.8 & -166 & 91.1 & 0.18 & 0.26 & 1.29 & 0.18 & 0.71 & N \\ 
 611 & 5 36 35.3 & 6 9 34 & 61.2 & 7369 & 5.6 & 28.9 & 15.3 & 158 & 96.9 & 0.19 & 0.28 & 3.56 & 0.08 & 1.64 & N \\ 
 612 & 5 36 35.7 & 6 19 12 & 79.0 & 4781 & 1.4 & 24.5 & 21.1 & -138 & 78.0 & 0.16 & 0.25 & 0.67 & 0.28 & 0.59 & N \\ 
 613 & 5 36 35.8 & 6 38 54 & 50.3 & 12881 & 3.2 & 45.4 & 21.3 & 47 & 128.1 & 0.26 & 0.28 & 6.07 & 0.06 & 1.21 & Y \\ 
 614 & 5 36 36.1 & 6 42 5 & 51.1 & 1856 & 2.0 & 20.0 & 7.2 & 93 & 48.6 & 0.10 & 0.20 & 0.43 & 0.17 & 1.57 & N \\ 
 615 & 5 36 37.0 & 6 43 10 & 49.7 & 3150 & 2.1 & 16.7 & 12.8 & 48 & 63.3 & 0.13 & 0.23 & 0.61 & 0.21 & 1.00 & N \\ 
 616 & 5 36 37.2 & 6 38 20 & 40.4 & 2250 & 1.4 & 20.0 & 9.3 & 89 & 53.5 & 0.11 & 0.21 & 0.36 & 0.24 & 0.99 & Y \\ 
 617 & 5 36 37.3 & 6 10 48 & 64.0 & 3319 & 3.7 & 19.0 & 13.7 & 90 & 65.0 & 0.13 & 0.16 & 0.95 & 0.07 & 1.45 & N \\ 
 618 & 5 36 37.3 & 6 41 1 & 50.4 & 4725 & 3.1 & 25.4 & 15.1 & 61 & 77.6 & 0.16 & 0.22 & 1.15 & 0.12 & 1.03 & N \\ 
 619 & 5 36 37.5 & 6 46 39 & 66.8 & 3600 & 1.7 & 17.7 & 15.3 & 58 & 67.7 & 0.14 & 0.34 & 0.84 & 0.35 & 1.13 & N \\ 
 620 & 5 36 37.6 & 6 3 45 & 62.3 & 2813 & 4.9 & 21.0 & 9.6 & 59 & 59.8 & 0.12 & 0.29 & 2.34 & 0.08 & 4.55 & N \\ 
 621 & 5 36 37.8 & 6 48 41 & 57.2 & 3206 & 1.4 & 29.1 & 14.6 & 137 & 63.9 & 0.13 & 0.17 & 0.71 & 0.10 & 1.14 & N \\ 
 622 & 5 36 38.0 & 6 39 54 & 68.5 & 5681 & 2.6 & 49.7 & 17.3 & 54 & 85.1 & 0.17 & 0.25 & 1.37 & 0.15 & 0.93 & Y \\ 
 623 & 5 36 38.5 & 6 13 34 & 61.9 & 16763 & 5.7 & 49.4 & 24.0 & -145 & 146.1 & 0.29 & 0.40 & 9.17 & 0.10 & 1.23 & N \\ 
 624 & 5 36 38.5 & 6 35 28 & 39.5 & 5175 & 1.5 & 34.4 & 15.5 & 73 & 81.2 & 0.16 & 0.32 & 0.85 & 0.38 & 0.67 & N \\ 
 625 & 5 36 38.5 & 6 43 50 & 61.3 & 4219 & 1.5 & 35.4 & 11.6 & -138 & 73.3 & 0.15 & 0.24 & 0.68 & 0.24 & 0.72 & N \\ 
 626 & 5 36 39.2 & 6 30 38 & 61.6 & 3825 & 1.4 & 30.0 & 14.4 & -161 & 69.8 & 0.14 & 0.28 & 0.27 & 0.74 & 0.34 & N \\ 
 627 & 5 36 39.7 & 6 34 54 & 45.2 & 1856 & 1.4 & 18.2 & 8.2 & 97 & 48.6 & 0.10 & 0.19 & 0.16 & 0.40 & 0.58 & N \\ 
 628 & 5 36 39.9 & 6 40 52 & 63.1 & 1631 & 1.8 & 11.8 & 10.2 & 94 & 45.6 & 0.09 & 0.18 & 0.17 & 0.33 & 0.75 & N \\ 
 629 & 5 36 40.1 & 6 13 38 & 41.6 & 29588 & 3.1 & 71.4 & 32.2 & 177 & 194.1 & 0.39 & 0.23 & 4.31 & 0.09 & 0.25 & Y \\ 
 630 & 5 36 41.0 & 6 22 44 & 65.3 & 1688 & 2.8 & 17.8 & 6.8 & -167 & 46.4 & 0.09 & 0.21 & 0.37 & 0.21 & 1.54 & N \\ 
 631 & 5 36 41.9 & 6 26 37 & 38.7 & 1631 & 3.7 & 16.9 & 8.9 & -156 & 45.6 & 0.09 & 0.24 & 1.53 & 0.07 & 6.73 & N \\ 
 632 & 5 36 42.4 & 6 18 20 & 66.1 & 11081 & 3.7 & 51.2 & 21.1 & 63 & 118.8 & 0.24 & 0.23 & 3.01 & 0.08 & 0.75 & N \\ 
 633 & 5 36 42.5 & 6 41 15 & 52.3 & 3994 & 2.3 & 25.8 & 11.8 & 70 & 71.3 & 0.14 & 0.22 & 0.69 & 0.19 & 0.80 & N \\ 
 634 & 5 36 42.6 & 6 20 33 & 54.9 & 2250 & 2.7 & 14.1 & 10.3 & 169 & 53.5 & 0.11 & 0.23 & 0.52 & 0.21 & 1.43 & N \\ 
 635 & 5 36 42.8 & 6 1 39 & 52.0 & 4781 & 1.4 & 46.3 & 17.3 & 112 & 78.0 & 0.16 & 0.20 & 0.60 & 0.19 & 0.53 & N \\ 
 636 & 5 36 42.9 & 6 1 57 & 60.0 & 3263 & 1.9 & 18.9 & 14.3 & 85 & 64.5 & 0.13 & 0.12 & 0.63 & 0.06 & 0.98 & N \\ 
 637 & 5 36 43.3 & 6 46 35 & 52.3 & 3994 & 1.9 & 20.8 & 16.4 & 143 & 71.3 & 0.14 & 0.16 & 0.60 & 0.12 & 0.69 & N \\ 
 638 & 5 36 43.7 & 6 21 25 & 66.3 & 4500 & 3.3 & 23.0 & 17.1 & 137 & 75.7 & 0.15 & 0.30 & 1.40 & 0.19 & 1.35 & N \\ 
 639 & 5 36 44.5 & 6 25 29 & 71.0 & 2925 & 1.8 & 21.1 & 12.5 & -166 & 61.0 & 0.12 & 0.19 & 0.21 & 0.41 & 0.39 & N \\ 
 640 & 5 36 44.7 & 6 42 53 & 55.2 & 2925 & 1.9 & 17.1 & 10.7 & 70 & 61.0 & 0.12 & 0.30 & 0.64 & 0.32 & 1.18 & N \\ 
 641 & 5 36 44.8 & 6 35 46 & 53.4 & 3544 & 3.3 & 21.2 & 11.4 & -141 & 67.2 & 0.13 & 0.24 & 0.88 & 0.16 & 1.22 & N \\ 
 642 & 5 36 44.8 & 6 44 15 & 53.2 & 6694 & 2.4 & 29.1 & 13.8 & 61 & 92.3 & 0.19 & 0.45 & 1.60 & 0.45 & 0.85 & N \\ 
 643 & 5 36 45.0 & 6 30 11 & 52.2 & 2475 & 2.4 & 16.3 & 9.7 & 73 & 56.1 & 0.11 & 0.47 & 0.48 & 0.97 & 1.12 & N \\ 
 644 & 5 36 45.2 & 6 6 21 & 63.3 & 8550 & 4.9 & 38.0 & 19.6 & -151 & 104.3 & 0.21 & 0.23 & 3.40 & 0.06 & 1.25 & N \\ 
 645 & 5 36 45.2 & 6 24 9 & 60.8 & 1519 & 3.5 & 16.6 & 6.7 & 93 & 44.0 & 0.09 & 0.20 & 0.60 & 0.12 & 2.96 & N \\ 
 646 & 5 36 45.6 & 6 17 48 & 37.6 & 9731 & 2.0 & 37.7 & 19.3 & -144 & 111.3 & 0.22 & 0.31 & 0.93 & 0.45 & 0.28 & N \\ 
 647 & 5 36 46.0 & 6 5 28 & 42.5 & 15469 & 1.8 & 33.0 & 31.3 & 104 & 140.3 & 0.28 & 0.52 & 1.88 & 0.76 & 0.28 & N \\ 
 648 & 5 36 46.1 & 6 21 22 & 59.3 & 4388 & 3.0 & 18.1 & 14.6 & 110 & 74.7 & 0.15 & 0.35 & 1.03 & 0.33 & 1.03 & N \\ 
 649 & 5 36 46.1 & 6 31 10 & 47.1 & 4613 & 3.8 & 24.4 & 12.5 & 161 & 76.6 & 0.15 & 0.34 & 1.59 & 0.21 & 1.48 & N \\ 
 650 & 5 36 46.2 & 6 15 22 & 63.0 & 4106 & 5.0 & 18.1 & 13.9 & 99 & 72.3 & 0.15 & 0.31 & 1.85 & 0.14 & 2.05 & N \\ 
 651 & 5 36 46.7 & 6 33 29 & 54.1 & 8044 & 3.3 & 66.9 & 21.1 & 96 & 101.2 & 0.20 & 0.37 & 1.94 & 0.27 & 0.78 & N \\ 
 652 & 5 36 46.8 & 6 25 26 & 60.7 & 3150 & 3.6 & 20.8 & 9.3 & 45 & 63.3 & 0.13 & 0.31 & 1.18 & 0.20 & 1.95 & N \\ 
 653 & 5 36 47.6 & 6 15 57 & 35.9 & 12825 & 2.0 & 43.9 & 26.9 & 52 & 127.8 & 0.26 & 0.37 & 1.12 & 0.59 & 0.22 & N \\ 
 654 & 5 36 47.6 & 6 19 50 & 41.1 & 13613 & 2.0 & 40.0 & 27.0 & 147 & 131.7 & 0.26 & 0.29 & 1.64 & 0.25 & 0.30 & N \\ 
 655 & 5 36 47.8 & 6 28 36 & 40.5 & 9844 & 4.0 & 48.4 & 15.8 & 49 & 112.0 & 0.22 & 0.41 & 5.27 & 0.13 & 1.57 & N \\ 
 656 & 5 36 48.1 & 6 26 11 & 74.4 & 6525 & 1.7 & 33.8 & 18.7 & 128 & 91.1 & 0.18 & 0.48 & 0.56 & 1.41 & 0.31 & N \\ 
 657 & 5 36 48.2 & 6 19 31 & 56.8 & 2925 & 1.6 & 24.2 & 9.2 & 67 & 61.0 & 0.12 & 0.20 & 0.21 & 0.44 & 0.38 & N \\ 
 658 & 5 36 48.9 & 6 35 15 & 43.3 & 3600 & 1.5 & 21.5 & 15.7 & 139 & 67.7 & 0.14 & 0.17 & 0.48 & 0.16 & 0.65 & N \\ 
 659 & 5 36 49.4 & 6 23 0 & 67.5 & 5906 & 3.7 & 29.4 & 14.5 & 141 & 86.7 & 0.17 & 0.27 & 2.11 & 0.12 & 1.35 & N \\ 
 660 & 5 36 49.5 & 6 2 34 & 63.8 & 5850 & 1.4 & 44.6 & 19.9 & 83 & 86.3 & 0.17 & 0.37 & 1.26 & 0.36 & 0.82 & N \\ 
 661 & 5 36 49.9 & 6 21 20 & 68.0 & 3206 & 3.3 & 17.3 & 14.8 & 60 & 63.9 & 0.13 & 0.19 & 0.79 & 0.11 & 1.26 & N \\ 
 662 & 5 36 50.0 & 6 39 52 & 49.7 & 4388 & 2.6 & 27.1 & 10.0 & 63 & 74.7 & 0.15 & 0.30 & 0.89 & 0.30 & 0.89 & N \\ 
 663 & 5 36 50.1 & 6 28 51 & 53.3 & 7425 & 4.0 & 34.0 & 13.3 & -140 & 97.2 & 0.20 & 0.37 & 3.57 & 0.14 & 1.62 & N \\ 
 664 & 5 36 52.8 & 6 41 7 & 50.8 & 3938 & 1.9 & 22.3 & 13.2 & 107 & 70.8 & 0.14 & 0.38 & 0.63 & 0.60 & 0.74 & N \\ 
 665 & 5 36 53.3 & 6 32 24 & 35.9 & 10350 & 2.1 & 40.1 & 17.7 & 102 & 114.8 & 0.23 & 0.37 & 2.46 & 0.24 & 0.68 & N \\ 
 666 & 5 36 53.5 & 6 17 16 & 70.0 & 3544 & 2.2 & 20.8 & 13.4 & 68 & 67.2 & 0.13 & 0.28 & 0.46 & 0.43 & 0.64 & N \\ 
 667 & 5 36 53.8 & 6 18 1 & 36.5 & 5625 & 1.8 & 25.8 & 18.6 & 71 & 84.6 & 0.17 & 0.28 & 0.62 & 0.40 & 0.43 & N \\ 
 668 & 5 36 54.1 & 6 33 47 & 66.0 & 7425 & 1.9 & 32.8 & 16.6 & 92 & 97.2 & 0.20 & 0.51 & 1.19 & 0.79 & 0.54 & N \\ 
 669 & 5 36 55.1 & 6 34 51 & 36.0 & 3488 & 2.6 & 17.2 & 12.2 & -152 & 66.6 & 0.13 & 0.39 & 1.17 & 0.32 & 1.65 & N \\ 
 670 & 5 36 55.3 & 6 19 17 & 72.7 & 3038 & 2.4 & 20.6 & 12.5 & 123 & 62.2 & 0.12 & 0.20 & 0.52 & 0.17 & 0.90 & N \\ 
 671 & 5 36 55.6 & 6 34 29 & 44.2 & 1575 & 2.0 & 12.7 & 8.8 & -178 & 44.8 & 0.09 & 0.24 & 0.29 & 0.35 & 1.33 & N \\ 
 672 & 5 36 55.7 & 6 31 52 & 48.4 & 7594 & 2.3 & 44.4 & 17.2 & 70 & 98.3 & 0.20 & 0.24 & 1.82 & 0.12 & 0.80 & N \\ 
 673 & 5 36 56.0 & 6 22 37 & 64.9 & 6469 & 2.4 & 24.6 & 17.0 & 53 & 90.8 & 0.18 & 0.28 & 2.16 & 0.12 & 1.21 & N \\ 
 674 & 5 36 57.2 & 6 35 20 & 94.0 & 2588 & 1.4 & 18.3 & 11.2 & 134 & 57.4 & 0.12 & 0.30 & 0.29 & 0.67 & 0.64 & N \\ 
 675 & 5 36 57.4 & 6 41 14 & 99.4 & 2531 & 1.5 & 19.1 & 10.0 & 165 & 56.8 & 0.11 & 0.24 & 0.28 & 0.47 & 0.63 & N \\ 
 676 & 5 36 57.5 & 6 40 48 & 43.0 & 2869 & 2.1 & 16.1 & 10.9 & 49 & 60.4 & 0.12 & 0.21 & 0.51 & 0.20 & 0.96 & N \\ 
 677 & 5 36 57.7 & 6 15 52 & 46.2 & 4106 & 1.5 & 25.2 & 16.5 & 100 & 72.3 & 0.15 & 0.27 & 0.63 & 0.32 & 0.70 & N \\ 
 678 & 5 36 58.5 & 6 36 24 & 53.4 & 2700 & 2.1 & 15.8 & 10.9 & 106 & 58.6 & 0.12 & 0.34 & 0.73 & 0.35 & 1.52 & N \\ 
 679 & 5 36 59.3 & 6 19 1 & 36.0 & 5906 & 2.1 & 34.3 & 21.6 & -155 & 86.7 & 0.17 & 0.28 & 1.12 & 0.22 & 0.72 & N \\ 
 680 & 5 36 59.6 & 6 29 0 & 77.0 & 3375 & 1.4 & 38.0 & 11.8 & 53 & 65.6 & 0.13 & 0.20 & 0.83 & 0.12 & 1.24 & N \\ 
 681 & 5 36 59.7 & 6 20 31 & 76.8 & 2250 & 1.4 & 22.5 & 11.3 & 141 & 53.5 & 0.11 & 0.27 & 0.26 & 0.57 & 0.70 & N \\ 
 682 & 5 37 0.2 & 6 39 2 & 41.2 & 3713 & 3.0 & 36.4 & 8.4 & 78 & 68.8 & 0.14 & 0.31 & 1.30 & 0.19 & 1.67 & N \\ 
 683 & 5 37 0.3 & 6 24 44 & 65.9 & 9844 & 2.3 & 45.9 & 22.6 & 88 & 112.0 & 0.22 & 0.33 & 3.29 & 0.14 & 0.98 & N \\ 
 684 & 5 37 0.6 & 6 24 58 & 74.1 & 3544 & 1.5 & 25.2 & 12.7 & 162 & 67.2 & 0.13 & 0.37 & 0.64 & 0.54 & 0.89 & N \\ 
 685 & 5 37 0.6 & 6 37 5 & 39.3 & 3544 & 3.3 & 15.2 & 14.1 & 47 & 67.2 & 0.13 & 0.30 & 3.90 & 0.06 & 5.37 & Y \\ 
 686 & 5 37 1.8 & 6 35 23 & 44.1 & 5400 & 3.7 & 24.3 & 16.7 & -160 & 82.9 & 0.17 & 0.34 & 3.07 & 0.12 & 2.25 & N \\ 
 687 & 5 37 2.3 & 6 39 5 & 52.0 & 3319 & 1.6 & 32.2 & 10.2 & 108 & 65.0 & 0.13 & 0.14 & 0.43 & 0.12 & 0.65 & N \\ 
 688 & 5 37 3.4 & 6 20 16 & 71.3 & 7144 & 1.7 & 28.4 & 16.5 & 159 & 95.4 & 0.19 & 0.63 & 1.81 & 0.80 & 0.87 & N \\ 
 689 & 5 37 3.7 & 6 17 54 & 34.7 & 5456 & 1.5 & 27.9 & 17.7 & -151 & 83.3 & 0.17 & 0.30 & 1.63 & 0.17 & 1.18 & N \\ 
 690 & 5 37 4.1 & 6 34 13 & 60.7 & 2306 & 1.4 & 15.6 & 10.8 & 72 & 54.2 & 0.11 & 0.25 & 0.24 & 0.56 & 0.62 & N \\ 
 691 & 5 37 5.5 & 6 23 43 & 69.4 & 5063 & 1.7 & 23.2 & 12.5 & 78 & 80.3 & 0.16 & 0.50 & 1.86 & 0.42 & 1.50 & N \\ 
 692 & 5 37 6.0 & 6 35 41 & 41.6 & 2700 & 3.5 & 16.0 & 11.8 & -157 & 58.6 & 0.12 & 0.26 & 1.20 & 0.12 & 2.49 & N \\ 
 693 & 5 37 6.9 & 6 27 22 & 69.2 & 4106 & 2.0 & 28.2 & 12.2 & -150 & 72.3 & 0.15 & 0.17 & 2.01 & 0.04 & 2.22 & N \\ 
 694 & 5 37 7.1 & 6 36 58 & 67.0 & 3319 & 1.4 & 21.8 & 14.4 & 140 & 65.0 & 0.13 & 0.25 & 0.74 & 0.21 & 1.13 & N \\ 
 695 & 5 37 8.5 & 6 26 2 & 64.7 & 8269 & 1.4 & 31.1 & 26.2 & 138 & 102.6 & 0.21 & 0.26 & 5.16 & 0.05 & 1.99 & N \\ 
 696 & 5 37 8.5 & 6 28 18 & 73.3 & 5738 & 1.8 & 21.7 & 18.4 & 159 & 85.5 & 0.17 & 0.46 & 2.79 & 0.25 & 1.86 & N \\ 
 697 & 5 37 8.9 & 6 44 40 & 55.4 & 8100 & 2.2 & 54.2 & 19.3 & 63 & 101.6 & 0.20 & 0.42 & 1.92 & 0.35 & 0.77 & N \\ 
 698 & 5 37 9.1 & 6 36 13 & 38.4 & 3319 & 3.3 & 17.5 & 12.3 & 142 & 65.0 & 0.13 & 0.32 & 1.71 & 0.15 & 2.59 & N \\ 
 699 & 5 37 9.9 & 6 38 41 & 65.2 & 4838 & 1.8 & 40.8 & 12.8 & -161 & 78.5 & 0.16 & 0.34 & 0.69 & 0.50 & 0.60 & N \\ 
 700 & 5 37 10.8 & 6 31 20 & 69.3 & 3881 & 1.8 & 27.2 & 10.6 & 88 & 70.3 & 0.14 & 0.27 & 1.70 & 0.12 & 2.04 & N \\ 
 701 & 5 37 11.5 & 6 41 43 & 44.4 & 2588 & 3.1 & 17.5 & 11.9 & 109 & 57.4 & 0.12 & 0.29 & 1.17 & 0.15 & 2.59 & N \\ 
 702 & 5 37 11.8 & 6 31 57 & 74.5 & 2813 & 1.5 & 19.7 & 11.1 & 88 & 59.8 & 0.12 & 0.22 & 1.19 & 0.09 & 2.32 & N \\ 
 703 & 5 37 12.3 & 6 39 29 & 52.5 & 3825 & 4.0 & 25.2 & 10.1 & -148 & 69.8 & 0.14 & 0.28 & 1.79 & 0.12 & 2.20 & N \\ 
 704 & 5 37 13.9 & 6 27 39 & 67.8 & 6131 & 1.6 & 32.6 & 18.8 & 76 & 88.4 & 0.18 & 0.42 & 1.98 & 0.29 & 1.20 & N \\ 
 705 & 5 37 14.3 & 6 46 47 & 51.3 & 2925 & 2.2 & 17.6 & 12.9 & -147 & 61.0 & 0.12 & 0.22 & 0.86 & 0.13 & 1.59 & N \\ 
 706 & 5 37 14.8 & 6 27 19 & 37.3 & 11869 & 1.7 & 40.3 & 20.0 & 122 & 122.9 & 0.25 & 0.42 & 4.95 & 0.17 & 1.11 & N \\ 
 707 & 5 37 14.8 & 6 33 9 & 51.0 & 1913 & 1.6 & 15.0 & 9.4 & -163 & 49.3 & 0.10 & 0.18 & 0.40 & 0.15 & 1.38 & N \\ 
 708 & 5 37 15.5 & 6 19 36 & 35.0 & 1406 & 1.7 & 14.2 & 6.0 & 145 & 42.3 & 0.08 & 0.21 & 0.29 & 0.23 & 1.61 & N \\ 
 709 & 5 37 15.7 & 6 18 53 & 37.7 & 4275 & 1.4 & 31.0 & 14.3 & 49 & 73.8 & 0.15 & 0.26 & 1.11 & 0.17 & 1.16 & N \\ 
 710 & 5 37 15.8 & 6 36 18 & 46.4 & 3881 & 1.6 & 25.7 & 15.8 & -166 & 70.3 & 0.14 & 0.21 & 0.63 & 0.20 & 0.75 & Y \\ 
 711 & 5 37 15.8 & 6 36 19 & 54.1 & 5681 & 1.7 & 24.7 & 17.5 & 81 & 85.1 & 0.17 & 0.44 & 1.38 & 0.45 & 0.94 & Y \\ 
 712 & 5 37 16.1 & 6 30 11 & 41.7 & 5231 & 1.5 & 27.5 & 17.4 & -151 & 81.6 & 0.16 & 0.20 & 1.42 & 0.09 & 1.09 & N \\ 
 713 & 5 37 16.3 & 6 34 33 & 66.9 & 5569 & 2.2 & 37.8 & 14.1 & 64 & 84.2 & 0.17 & 0.27 & 1.48 & 0.15 & 1.03 & N \\ 
 714 & 5 37 16.3 & 6 46 28 & 57.9 & 7594 & 1.9 & 32.9 & 21.1 & 85 & 98.3 & 0.20 & 0.45 & 1.63 & 0.46 & 0.71 & N \\ 
 715 & 5 37 17.5 & 6 30 0 & 23.7 & 3544 & 1.7 & 26.1 & 11.1 & 83 & 67.2 & 0.13 & 0.39 & 0.76 & 0.51 & 1.04 & N \\ 
 716 & 5 37 17.5 & 6 33 23 & 73.9 & 4500 & 1.5 & 25.3 & 15.5 & -178 & 75.7 & 0.15 & 0.27 & 1.12 & 0.19 & 1.08 & N \\ 
 717 & 5 37 18.1 & 6 40 18 & 55.1 & 3488 & 3.8 & 17.4 & 12.8 & -167 & 66.6 & 0.13 & 0.22 & 1.73 & 0.07 & 2.44 & N \\ 
 718 & 5 37 18.6 & 6 46 13 & 50.2 & 2419 & 1.9 & 18.8 & 12.0 & 112 & 55.5 & 0.11 & 0.18 & 0.79 & 0.09 & 1.94 & N \\ 
 719 & 5 37 19.0 & 6 44 4 & 45.8 & 2981 & 2.2 & 19.7 & 11.5 & 155 & 61.6 & 0.12 & 0.19 & 0.80 & 0.10 & 1.43 & N \\ 
 720 & 5 37 19.1 & 6 37 16 & 40.7 & 5006 & 1.7 & 41.3 & 16.6 & 102 & 79.8 & 0.16 & 0.16 & 1.18 & 0.07 & 0.97 & N \\ 
 721 & 5 37 20.2 & 6 44 19 & 40.9 & 4444 & 1.9 & 23.4 & 16.6 & 156 & 75.2 & 0.15 & 0.19 & 1.08 & 0.10 & 1.06 & N \\ 
 722 & 5 37 20.5 & 6 34 60 & 39.0 & 3263 & 1.4 & 28.3 & 15.4 & 119 & 64.5 & 0.13 & 0.37 & 0.83 & 0.41 & 1.29 & N \\ 
 723 & 5 37 21.8 & 6 36 33 & 70.0 & 8325 & 1.4 & 32.5 & 21.6 & -138 & 103.0 & 0.21 & 0.69 & 2.61 & 0.71 & 1.00 & N \\ 
 724 & 5 37 22.2 & 6 47 43 & 59.9 & 6075 & 2.2 & 21.1 & 17.0 & 108 & 87.9 & 0.18 & 0.35 & 1.66 & 0.25 & 1.02 & N \\ 
 725 & 5 37 22.5 & 6 36 51 & 36.1 & 10519 & 2.8 & 35.6 & 19.9 & 138 & 115.7 & 0.23 & 0.39 & 5.17 & 0.13 & 1.39 & N \\ 
 726 & 5 37 22.9 & 6 41 43 & 52.9 & 8888 & 2.3 & 33.7 & 19.9 & 143 & 106.4 & 0.21 & 0.47 & 3.25 & 0.27 & 1.13 & N \\ 
 727 & 5 37 22.9 & 6 45 32 & 58.2 & 6356 & 1.8 & 23.4 & 22.0 & -161 & 90.0 & 0.18 & 0.30 & 1.57 & 0.19 & 0.90 & N \\ 
 728 & 5 37 25.0 & 6 47 4 & 48.2 & 5006 & 1.7 & 22.2 & 20.1 & 68 & 79.8 & 0.16 & 0.26 & 1.44 & 0.14 & 1.19 & N \\ 
 729 & 5 37 26.8 & 6 43 54 & 56.9 & 6638 & 1.8 & 38.6 & 15.3 & 174 & 91.9 & 0.18 & 0.27 & 2.00 & 0.13 & 1.08 & N \\ 
 730 & 5 37 27.3 & 6 39 7 & 37.2 & 4331 & 1.8 & 25.2 & 12.3 & 56 & 74.3 & 0.15 & 0.18 & 1.20 & 0.08 & 1.23 & N \\ 
 731 & 5 37 27.6 & 6 44 32 & 84.2 & 3263 & 1.8 & 15.8 & 11.6 & 88 & 64.5 & 0.13 & 0.41 & 0.79 & 0.51 & 1.23 & N \\ 
 732 & 5 37 28.9 & 6 39 5 & 42.9 & 5963 & 1.8 & 25.6 & 16.0 & 89 & 87.1 & 0.17 & 0.42 & 2.18 & 0.27 & 1.38 & N \\ 
 733 & 5 37 29.7 & 6 44 48 & 41.4 & 11588 & 1.8 & 32.7 & 25.4 & 50 & 121.5 & 0.24 & 0.44 & 5.20 & 0.18 & 1.21 & N \\ 
 734 & 5 37 30.4 & 6 42 3 & 33.4 & 2250 & 2.2 & 17.2 & 9.2 & 164 & 53.5 & 0.11 & 0.19 & 0.96 & 0.08 & 2.62 & N \\ 
 735 & 5 37 31.1 & 6 34 59 & 41.0 & 3881 & 1.8 & 23.2 & 15.4 & 80 & 70.3 & 0.14 & 0.24 & 1.27 & 0.12 & 1.53 & N \\ 
 736 & 5 37 33.8 & 6 36 51 & 39.5 & 9675 & 2.9 & 33.5 & 20.8 & -169 & 111.0 & 0.22 & 0.30 & 3.40 & 0.12 & 1.04 & N \\ 
 737 & 5 37 36.8 & 6 45 59 & 42.0 & 2869 & 1.8 & 22.3 & 10.6 & 53 & 60.4 & 0.12 & 0.21 & 0.94 & 0.11 & 1.78 & N \\ 
 738 & 5 37 37.5 & 6 34 40 & 39.3 & 5906 & 1.7 & 30.7 & 14.8 & 117 & 86.7 & 0.17 & 0.25 & 2.38 & 0.09 & 1.52 & N \\ 
 739 & 5 37 38.2 & 6 45 16 & 67.3 & 2869 & 1.7 & 19.7 & 13.1 & 127 & 60.4 & 0.12 & 0.23 & 0.53 & 0.22 & 1.01 & N \\ 
 740 & 5 37 38.5 & 6 42 59 & 34.2 & 6188 & 2.4 & 27.1 & 14.7 & -165 & 88.8 & 0.18 & 0.36 & 3.49 & 0.13 & 2.09 & N \\ 
 741 & 5 37 41.2 & 6 36 48 & 38.5 & 6525 & 2.9 & 31.9 & 17.5 & 82 & 91.1 & 0.18 & 0.25 & 1.43 & 0.15 & 0.79 & N \\ 
 742 & 5 37 42.8 & 6 44 21 & 62.9 & 4444 & 1.4 & 30.7 & 13.9 & 106 & 75.2 & 0.15 & 0.21 & 1.36 & 0.09 & 1.33 & N \\ 
 743 & 5 37 43.3 & 6 45 29 & 43.2 & 4163 & 1.7 & 27.1 & 12.6 & -140 & 72.8 & 0.15 & 0.42 & 1.07 & 0.46 & 1.16 & N \\ 
 744 & 5 37 45.4 & 6 39 24 & 42.9 & 2250 & 1.9 & 16.8 & 10.3 & 146 & 53.5 & 0.11 & 0.19 & 0.77 & 0.09 & 2.10 & N \\ 
 745 & 5 37 45.9 & 6 42 32 & 43.6 & 5794 & 2.1 & 30.6 & 21.2 & -164 & 85.9 & 0.17 & 0.48 & 1.75 & 0.43 & 1.16 & N \\ 
 746 & 5 37 47.2 & 6 40 41 & 31.5 & 3263 & 1.9 & 35.2 & 8.6 & 121 & 64.5 & 0.13 & 0.19 & 0.58 & 0.14 & 0.91 & N \\ 
 \hline 

